Gaussian Approximation of Convex Sets by Intersections of Halfspaces

We study the approximability of general convex sets in $\mathbb{R}^n$ by intersections of halfspaces, where the approximation quality is measured with respect to the standard Gaussian distribution $N(0,I_n)$ and the complexity of an approximation is the number of halfspaces used. While a large body of research has considered the approximation of convex sets by intersections of halfspaces under distance metrics such as the Lebesgue measure and Hausdorff distance, prior to our work there has not been a systematic study of convex approximation under the Gaussian distribution. We establish a range of upper and lower bounds, both for general convex sets and for specific natural convex sets that are of particular interest. Our results demonstrate that the landscape of approximation is intriguingly different under the Gaussian distribution versus previously studied distance measures. For example, we show that $2^{\Theta(\sqrt{n})}$ halfspaces are both necessary and sufficient to approximate the origin-centered $\ell_2$ ball of Gaussian volume 1/2 to any constant accuracy, and that for $1 \leq p < 2$, the origin-centered $\ell_p$ ball of Gaussian volume 1/2 can be approximated to any constant accuracy as an intersection of $2^{\widetilde{O}(n^{3/4})}$ many halfspaces. These bounds are quite different from known approximation results under more commonly studied distance measures. Our results are proved using techniques from many different areas. These include classical results on convex polyhedral approximation, Cram\'er-type bounds on large deviations from probability theory, and -- perhaps surprisingly -- a range of topics from computational complexity, including computational learning theory, unconditional pseudorandomness, and the study of influences and noise sensitivity in the analysis of Boolean functions.

==> sections/ball-approx.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Approximating the $\ell_2$-Ball}
\label{sec:ball-apx}


\subsection{An Upper Bound}
\label{subsec:nazarov}




\begin{lemma}
	
\end{lemma}


\subsection{Lower Bounds}
\label{subsec:ball-lbs}



\subsubsection{Constant-Error Approximators}
\label{subsec:convex-inf-lb}





\subsubsection{Small-Error Approximators}
\label{subsec:hausdorff-lb}

I guess here we can include the small-error lower bound obtained via the symmetric distance approximation lower bounds?




==> sections/convex-influences-backup.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Lower Bounds for the $\ell_2$-Ball (and more) via Convex Influences}
\label{sec:conv-inf}

Taking $\eps$ to be a sufficiently small constant in \Cref{lb:non-explicit-convex}, we can infer the existence of some convex set in $\R^n$ such that $2^{\Omega(\sqrt{n})}$ halfspaces are required for any $\eps$-approximator, but that result did not let us conclude that any particular convex set is hard to approximate.

In this section we show that the $\ell_2$ ball $B:=B(\sqrt{n})$ of radius $\sqrt{n}$ is in fact such a hard-to-approximate convex set:  

\begin{theorem} \label{thm:ball-conv-inf-lb}
	Any intersection of halfspaces that approximates $B(\sqrt{n})$ to error $\red{TODO}$ must have at least $2^{\Omega(\sqrt{n})}$ facets. 
\end{theorem}

\Cref{thm:ball-conv-inf-lb} in turn implies that the upper bound obtained in~\Cref{sec:nazarov-ub} is tight in the constant error regime, up to constant factors in the exponent. Our bound will crucially make use of the notion of \emph{convex influence} introduced by~\cite{DNS21itcs,DNS22}. More generally, we prove a lower bound on the number of facets required to approximate any convex set whose convex influence is asymptotically maximal up to constant multiplicative factors (cf.~\Cref{thm:high-influence-lb}); see~\Cref{subsec:convex-influence-lower-bound} for more on this.

\begin{remark}
We note that the results of \Cref{sec:noise-sensitivity} do not apply to $B$, since $B$ is well known to be highly noise stable. In more detail, \cite{Ball:93} showed that every origin-centered ball $B(r) \subseteq \R^n$ of any radius $r$ has Gaussian surface area $\GSA(B(r)) \leq 1/\sqrt{\pi} + o_n(1)$, and it is known (see e.g.~Corollary~14 of \cite{KOS:08}) that for any noise rate $\delta$ and any convex set $K$, we have $\GNS_\delta(K) \leq \sqrt{\pi} \cdot \sqrt{\delta} \cdot \GSA(K).$
\end{remark}

\subsection{Convex Influences}
\label{subsec:convex-influence}


The following notion was introduced in \cite{DNS21itcs,DNS22} as an analogue of the well-studied notion of \emph{influence of a variable on a Boolean function} (cf. Chapter~2 of \cite{odonnell-book}). 

\begin{definition} \label{def:convex-influence}
	Given a convex set $K\sse\R^n$ with $0^n\in K$, the \emph{convex influence of a direction $v\in \S^{n-1}$ on $K$} is defined as
	\[\Inf_v[K] := \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{{1 - \abra{\bx, v}^2}}},\]
{where $K(\cdot)$ is the 0/1-valued indicator function of the convex set $K$.}
	Furthermore, we define the \emph{total convex influence of $K$} as 
	\[\TInf[K] := \sum_{i=1}^n \Inf_{e_i}[K] = \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{{n- \|\bx\|^2}}}.\]
\end{definition}

We note that the definitions of $\Inf_{e_i}[K]$ and $\TInf[K]$ as defined in \cite{DNS22} include an additional multiplicative factor of ${1}/{\sqrt{2}}$ that we omit here. 
The total convex influence as defined above can be operationally understood as capturing the rate of growth of the Gaussian measure of a convex set under dilations. More formally, we have the following: 

\begin{proposition}[Dilation formulation of convex influence] \label{prop:inf-dilation}
	Given $K\sse\R^n$ with $0^n\in K$, we have 
	\[\TInf[K] = \lim_{\delta\to0}\frac{\vol\pbra{(1+\delta)K} - \vol(K)}{\delta}.\]
\end{proposition}

Note that if $K\sse\R^n$ is convex with $0^n\in K$, then $\TInf[K]$ is non-negative. \Cref{prop:inf-dilation} is analogous to the well-known Margulis--Russo lemma \cite{Margulis:74,Russo:78} from the analysis of Boolean functions, and a proof of it can be found in Appendix~A of \cite{De2021}. We note that a similar ``dilation formulation'' holds for the convex influence of a single direction $v\in \S^{n-1}$ on $K$, although we will not require it here. 

We will use the following alternative formulation of the total convex influence of a convex set, which was communicated to us by Joe Neeman~\cite{neeman:comm}:

\begin{lemma}[Influence via a surface integral] \label{lem:neeman}
	Given {a measurable set} $K\sse\R^n$ with $0^n\in K$ and a direction $v\in \S^{n-1}$, we have 
	\begin{equation*}
		\TInf[K] = \int_{\partial K} \abra{x, \nu_x}\cdot\phi(x)\,d\sigma(x)
	\end{equation*}
	where $\nu_x$ denotes the unit normal to $\partial K$ at $x$.
\end{lemma}

\begin{proof}
	The proof is a straightforward computation using integration by parts. Recall that via \Cref{def:convex-influence}, we have \rnote{Starting from the third equation below I didn't understand the rest of the proof but I'm sure you can convince me that it is okay}
\begin{align}
	\TInf[K] &= \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{\frac{n- \|\bx\|^2}{\sqrt{2}}}} \nonumber \\
	&= \int_K (n - \|x\|^2)\cdot\phi(x)\,dx \nonumber\\
	&= \int_K \calL\pbra{\frac{\|x\|^2}{2}}\cdot\phi(x)\,dx  \nonumber\\
	\intertext{where for a function $f:\R^n\to\R$ we define $\calL(f) := \Delta f - \abra{\nabla f, \nabla({\|x\|^2}/{2})}$. Integrating by parts then gives}
	\TInf[K] &= \int_{\partial K} \abra{x, \nu_x} \cdot \phi(x)\,d\sigma(x),\nonumber
\end{align}
completing the proof.
\end{proof}

\begin{remark}
	We note that the surface integral formulation of total convex influence can be viewed as analogous to the fact that the total influence of a Boolean function is equal to its average sensitivity (cf. Chapter 2 of~\cite{odonnell-book}). Although we will not require it for our purposes, we note that a similar formulation holds for the convex influence of a direction $v\in \S^{n-1}$ on $K$:
	\begin{equation*} \label{eq:neeman}
		\Inf_v[K] = \int_{\partial K} \abra{x, v}\cdot\abra{\nu_x, v}\cdot\phi(x)\,d\sigma(x)
	\end{equation*}
	where as before $\nu_x$ denotes the unit normal to $\partial K$ at $x$.
\end{remark}

\subsection{Bounds on the Convex Influence of Polytopes}
\label{sec:influence-structural-analogs}

%In this section, we obtain bounds on the convex influence of polytopes which suggest an analogy between Boolean CNF formulas and intersections of halfspaces which may be of independent interest. \Cref{prop:convex-boppana} will later be used in \Cref{subsec:convex-influence-lower-bound} to lower bound the number of facets needed to $0.001$-approximate the $\ell_2$-ball of volume $1/2$; \Cref{prop:influence-width-ub,prop:size-to-width} will not directly be linked to polytope approximation, and so we defer their proofs to \Cref{appendix:polytope-influence-bounds}.

We first obtain an upper bound on the total convex influence of an intersection of halfspaces in terms of the number of halfspaces. An analogous statement for CNF formulas over $\zo^n$, {showing that the influence of any $s$-clause CNF is at most $O(\log s)$,} was first given by Boppana~\cite{Boppana1997} using the technique of random restrictions~\cite{Hastad:86}. \footnote{In fact, Boppana~\cite{Boppana1997} obtains an upper bound of $O(\log^{d-1}(s))$ on the total influence of functions computed by depth-$d$ size-$s$ circuits.} The proof of \Cref{prop:convex-boppana} is a straightforward computation inspired by the proof of \Cref{thm:nazarov} due to Nazarov; we give a self-contained proof of \Cref{prop:convex-boppana} below (see~\cite{ball-lecture} for a proof sketch of Nazarov's bound).

\begin{proposition}[H\aa stad--Boppana analogues]
\label{prop:convex-boppana}
	Let $K \sse\R^n$ be an intersection of $s$ halfspaces. Then 
	\[\TInf[K] \leq O(\log s) + 1.\]
\end{proposition}

\begin{proof}[Proof of~\Cref{prop:convex-boppana}]
	When $s = 1$, the bound follows from an explicit calculation. So we let $K = \bigcap_{i=1}^s H_i$ for $s > 1$ where each $H_i$ is a halfspace of the form
	\[H_i := \cbra{x\in\R^n : \abra{x,v_i} \leq \theta_i}\]
	where $v_i \in \S^{n-1}$ for $i\in[s]$.
	Using \Cref{lem:neeman}, we have
	\begin{align}
		\TInf[K] &= \int_{\partial K} \abra{x,\nu_x}\cdot\phi(x)\,d\sigma(x) \nonumber\\
		&= \sum_{i=1}^s \pbra{\int_{\partial(H_i\cap K)} \abra{x,\nu_x}\cdot\phi(x)\,d\sigma(x)} \nonumber \\
		&= \sum_{i=1}^s \theta_i\cdot\GSA(H_i \cap K) \nonumber \\
		&= \sum_{\substack{i \in [s] \\ \theta_i \leq 10\sqrt{\log s}}} \theta_i\cdot\GSA(H_i \cap K) + \sum_{\substack{j \in [s] \\ \theta_j > 10\sqrt{\log s}}} \theta_j\cdot\GSA(H_j \cap K) 
		\label{eq:bop-sum}
	\end{align}
	where we used \Cref{eq:gsa-def} in the third equality. We will control each term in \Cref{eq:bop-sum} separately. Note that 
	\begin{equation} \label{eq:bop-sum-1}
		\sum_{\substack{i \in [s] \\ \theta_i \leq 10\sqrt{\log s}}} \theta_i\cdot\GSA(H_i \cap K) \leq 10\sqrt{\log s}\cdot \sum_{i=1}^s \GSA(H_i\cap K) \leq 10\log s,
	\end{equation}
	where the final inequality is due to Nazarov's bound on GSA (\Cref{thm:nazarov}). Note also that 
	\begin{align}
		\sum_{\substack{j \in [s] \\ \theta_j > 10\sqrt{\log s}}} \theta_j\cdot\GSA(H_j \cap K) &\leq \sum_{\substack{j \in [s] \\ \theta_j > 10\sqrt{\log s}}} \theta_j \cdot e^{-\theta_j^2/2}\nonumber\\
		& \leq s\cdot\max_{j : \theta_i > 10\sqrt{\log s}} \cbra{\theta_j\cdot e^{-\theta_j^2/2}}. \nonumber \\
		\intertext{Note that $xe^{-x^2/2}$ is a decreasing function for $x\geq 1$, and as $s >1$, it follows that $\theta_j\cdot e^{-\theta_j^2/2}$ is maximized for $\theta_j = 10\sqrt{\log s}$ which lets us write }
		& \leq O\pbra{\frac{s\sqrt{\log s}}{s^{50}}}. \label{eq:bop-sum-2}
	\end{align}
	The result follows from \Cref{eq:bop-sum,eq:bop-sum-1,eq:bop-sum-2}.
\end{proof}

\subsubsection{Digression} Let us continue to explore the analogy between intersections of halfspaces over $\R^n$ and CNF formulas over the Boolean hypercube. In addition to the size of a CNF, another natural complexity measure associated to a CNF is the \emph{width} of the CNF, which is the maximum number of literals in any clause of the CNF. The following proposition is analogous to the well-known fact that the total influence of a CNF of width $w$ is at most $O(w)$ (cf. Proposition 4.7 of~\cite{odonnell-book}; see~\cite{Amano-dnf} for the sharp constant). 

\begin{proposition} \label{prop:influence-width-ub}
	Let $K\sse\R^n$ be an intersection of $s$ halfspaces of the form 
	\[
	K = \bigcap_{i=1}^s H_i 
	\qquad\text{where}\qquad 
	H_i := \{x\in\R^n : \abra{x,v_i} \leq w\}
	\]
	for unit vectors $v_i \in \S^{n-1}$, and furthermore suppose $0^n\in K$.  Then we have 
	\[\TInf[K] \leq O(w^2).\]
\end{proposition}

{It is folklore that any $s$-clause CNF over $\zo^n$ can be $\eps$-approximated by a CNF in which each clause contains at most $\log(s/\eps)$ literals.  The following proposition gives an analogous result for intersections of halfspaces:}
% also straightforward to show that intersections of a small number of halfspaces can be well-approximated by intersections of not-too-wide halfspaces as well:

\begin{proposition} \label{prop:size-to-width}
	Let $K\sse\R^n$ be an intersection of $s$ halfspaces. For any $\eps >0$, there exists a set $L \sse\R^n$ which is an intersection of at most $s$ halfspaces $\{H_i\}$ where each $H_i$ is of the form
	\[ H_i := \cbra{x\in\R^n : \abra{x,v_i} \leq w}, \qquad\text{where}~w^2 = O\pbra{\log\pbra{\frac{s}{\epsilon}}},\]
	which satisfies $\dG(K, L) \leq \eps$.
\end{proposition}

As \Cref{prop:influence-width-ub,prop:size-to-width} will not be directly used in the remainder of this section, we defer their proofs to~\Cref{appendix:polytope-influence-bounds}.


\subsection{Lower Bounds for Approximating Convex Sets with Maximal Influence}
\label{subsec:convex-influence-lower-bound}

We finally establish the following lower bound on approximating sets with maximal convex influence:

\begin{theorem} \label{thm:high-influence-lb}
	Suppose $K\sse\R^n$ is a convex set with $\TInf[K] = \Theta(\sqrt{n})$. There exist absolute constants $0< c_0, c_1 < 1$ such that any polytope that $c_0$-approximates $K$ must have at least
	$2^{c_1\sqrt{n}}~\text{halfspaces}.$
\end{theorem}

\begin{proof}
	Note that it suffices to show the following:
	\begin{equation} \label{eq:inf-lb-goal}
		\text{If}~\dG(L,K) \leq c_0,~\text{then}~\TInf[L] = \Omega(\sqrt{n}).
	\end{equation}
	Indeed, with \Cref{eq:inf-lb-goal} in hand, it follows that if $L$ has $2^{c_1\sqrt{n}}$ halfspaces, it follows from \Cref{prop:convex-boppana} that
	\[\TInf[L] \leq c_1\sqrt{n} + 1\] 
	which contradicts~\Cref{eq:inf-lb-goal} for a sufficiently small constant $c_1$. 
	
	\Cref{eq:inf-lb-goal} is in fact immediate from the proof of Theorem~A.1 from~\cite{o2007approximation}, but we give an arguably simpler argument below for the reader's convenience. 
	Our proof will make use of the Hermite basis; we refer the reader to~\Cref{appendix:hermite} for a primer on Hermite analysis over the Gaussian measure. 
	Writing $e_i \in \R^n$ for the standard basis vector along the $i^\text{th}$ coordinate direction, we have that 
	\[\Inf_{e_i}[K] = \sqrt{2}\cdot\wt{K}(2e_i).\]
	We refer the reader to~\cite{DNS22} for a proof of this fact.
	Let $\alpha(K)$ be the vector of the convex influences of $K$ along the $n$ coordinate directions scaled by a factor of $2^{-1/2}$, i.e. 
	\[\alpha(K) := \pbra{\wt{K}(2e_1), \ldots, \wt{K}(2e_n)}\]
	with $\alpha(L)$ defined similarly. Now
	\begin{align*}
		\|\alpha(K) - \alpha(L)\|^2 &= \sumi (\wt{K}(2e_i) - \wt{L}(2e_i))^2\\
		&\leq \sum_{\alpha\in\N^n} (\wt{K}(\alpha) - \wt{L}(\alpha))^2 \\
		&= \Ex_{\bx\sim N(0,I_n)}\sbra{(K(\bx) - L(\bx))^2} \\
		&\leq c_0,
	\end{align*}
	where the penultimate equality relies on Parseval's formula (cf.~\Cref{appendix:hermite}) and the final inequality is due to $L$ being a $c_0$-approximator to $K$. \red{TODO: Finish this.}
\end{proof}

As a consequence of \Cref{thm:high-influence-lb}, we immediately obtain lower bounds for approximating the $\ell_2$ and $\ell_1$ balls of Gaussian measure $\approx 1/2$ as well as for Nazarov's body~\cite{Nazarov:03}:

\begin{example}[$\ell_2$ ball] \label{eg:ball-conv-inf}
	Example~13 of~\cite{DNS22} establishes that 
\[\TInf[B(\sqrt{n})] = \Theta(\sqrt{n}).\]
Together with~\Cref{thm:high-influence-lb}, this immediately implies that any $0.01$-approximation to $B(\sqrt{n})$ requires {$2^{\Omega(\sqrt{n})}$} facets. This in turn implies that \Cref{thm:de-nazarov} is tight up to constant factors when $\eps = 0.01$. 
\end{example}

\begin{examples}[Cross-polytope] \label{eg:cross-polytope-inf}
	Let $B_1$ be the cross-polytope, i.e. the set
	\[B_1 := \cbra{x\in\R^n : \|x\|_1 \leq\sqrt{\frac{2}{\pi}}n}.\]
	Note that $B_1$ is an intersection of $2^n$ halfspaces, and recall  from~\Cref{subsec:ell-1-warmup} that $\vol(B_1) = 1/2 \pm o_n(1)$. 
	By the Gaussian isoperimetric inequality, we have that $\GSA(B_1) = \Omega(1)$, and so using \Cref{lem:neeman} we have
	\[\TInf[B_1] = \sqrt{\frac{2}{\pi}n}\cdot\GSA(B_1) = \Omega(\sqrt{n}).\]
	Together with~\Cref{thm:high-influence-lb}, this immediately implies that any $0.01$-approximation to $B(\sqrt{n})$ requires {$2^{\Omega(\sqrt{n})}$} facets. (Recall from~\Cref{subsec:ell-1-warmup} that $B_1$ can be $0.01$-approximated using $2^{\Theta(n^{3/4})}$ halfspaces.)
\end{examples}

\begin{example}[Nazarov's body] \label{eg:naz-conv-inf}
	Nazarov~\cite{Nazarov:03} established (via a probabilistic argument) the existence of a polytope $K$ with $2^{\Theta(\sqrt{n})}$ facets, each at Euclidean distance $\Theta(n^{1/4})$ from the origin, with $\GSA(K) = \Theta(n^{1/4})$. It follows from \Cref{lem:neeman} that
	\[\TInf[K] = \Theta(n^{1/4}) \cdot \GSA(K) = \Theta(\sqrt{n}).\]
	\Cref{thm:high-influence-lb} thus implies that Nazarov's body cannot be approximated by a polytope with significantly fewer facets. 
\end{example}











==> sections/convex-influences-sort-of-safe-11-10-10pm.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Lower Bounds for the $\ell_1$ and $\ell_2$ Balls (and More) via Convex Influences}
\label{sec:conv-inf}

Taking $\eps$ to be a sufficiently small constant in \Cref{lb:non-explicit-convex}, we can infer the existence of some convex set in $\R^n$ such that $2^{\Omega(\sqrt{n})}$ halfspaces are required for any $\eps$-approximator, but that result does not let us conclude that any particular convex set is hard to approximate.

In this section we show that the $\ell_1$ and $\ell_2$ balls $B_1$ and $B_2$ (defined in  \Cref{eq:Bp}) are each hard to approximate:

\begin{theorem} \label{thm:ball-conv-inf-lb}
	Any intersection of halfspaces that approximates $B_2$ to error $\eps$ must have at least $2^{\Omega(\sqrt{n})}$ facets, for some absolute positive constant $\eps > 0.$
	{The same is true for $B_1$.}
\end{theorem}

\Cref{thm:ball-conv-inf-lb} implies that the upper bound obtained in~\Cref{sec:nazarov-ub} is tight in the constant error regime, up to constant factors in the exponent. 

Our proof of \Cref{thm:ball-conv-inf-lb} will crucially make use of the notion of \emph{convex influence} which was introduced by~\cite{DNS21itcs,DNS22}. More generally, we prove a lower bound on the number of facets required to approximate any \red{symmetric}\footnote{Recall that a set $K\sse\R^n$ is \emph{symmetric} if $x\in K$ implies $-x\in K$.}  convex set whose convex influence is asymptotically maximal up to constant multiplicative factors (cf.~\Cref{thm:high-influence-lb}); see~\Cref{subsec:convex-influence-lower-bound} for more on this.

\begin{remark}
We note that the results of \Cref{sec:noise-sensitivity} do not apply to $B_2$, since $B_2$ is well known to be highly noise stable. In more detail, \cite{Ball:93} showed that every origin-centered ball $B(r) \subseteq \R^n$ of any radius $r$ has Gaussian surface area $\GSA(B(r)) \leq 1/\sqrt{\pi} + o_n(1)$, and it is known (see e.g.~Corollary~14 of \cite{KOS:08}) that for any noise rate $\delta$ and any convex set $K$, we have $\GNS_\delta(K) \leq \sqrt{\pi} \cdot \sqrt{\delta} \cdot \GSA(K).$
It can similarly be shown that $B_1$ is also too noise-stable for the results of \Cref{sec:noise-sensitivity} to apply.
%\rnote{Are we okay saying this? Since we mention that those earlier results don't apply to $B_2$ maybe we should also say they don't apply to $B_1$. Surely $B_1$ is noise stable, right - I think that at a low noise rate $B_1$ will just look like whatever boundary hyperplane you happen to be close to, no? If we're not comfortable saying this we can delete this red sentence.}
\end{remark}

\subsection{Convex Influences}
\label{subsec:convex-influence}


The following notion was introduced in \cite{DNS21itcs,DNS22} as an analogue of the well-studied notion of \emph{influence of a variable on a Boolean function} (cf. Chapter~2 of \cite{odonnell-book}). 

\begin{definition} \label{def:convex-influence}
	Given a convex set $K\sse\R^n$ with $0^n\in K$, the \emph{convex influence of a direction $v\in \S^{n-1}$ on $K$} is defined as
	\[\Inf_v[K] := \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{{1 - \abra{\bx, v}^2}}},\]
{where $K(\cdot)$ is the 0/1-valued indicator function of the convex set $K$.}
	We further define the \emph{total convex influence of $K$} as 
	\[\TInf[K] := \sum_{i=1}^n \Inf_{e_i}[K] = \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{{n- \|\bx\|^2}}}.\]
\end{definition}

We note that the definitions of $\Inf_{v}[K]$ and $\TInf[K]$ as defined in \cite{DNS22} include an additional multiplicative factor of ${1}/{\sqrt{2}}$ that we omit here. 
The total convex influence as defined above can be understood as capturing the rate of growth of the Gaussian measure of a convex set under dilations. More formally, we have the following:

\begin{proposition}[Dilation formulation of convex influence] \label{prop:inf-dilation}
	Given $K\sse\R^n$ with $0^n\in K$, we have 
	\[\TInf[K] = \lim_{\delta\to0}\frac{\vol\pbra{(1+\delta)K} - \vol(K)}{\delta}.\]
\end{proposition}

Note that if $K\sse\R^n$ is convex with $0^n\in K$, then $\TInf[K]$ is non-negative. \Cref{prop:inf-dilation} is analogous to the well-known Margulis--Russo lemma \cite{Margulis:74,Russo:78} from the analysis of Boolean functions, and a proof of it can be found in Appendix~A of \cite{De2021}. We note that a similar ``dilation formulation'' holds for the convex influence of a single direction $v\in \S^{n-1}$ on $K$, although we will not require it here. 

We will use the following alternative formulation of the total convex influence of a convex set, which was communicated to us by Joe Neeman~\cite{neeman:comm}:

\begin{lemma}[Influence via a surface integral] \label{lem:neeman}
	Given {a measurable set} $K\sse\R^n$ with $0^n\in K$ and a direction $v\in \S^{n-1}$, we have 
	\begin{equation*}
		\TInf[K] = \int_{\partial K} \abra{x, \nu_x}\cdot\phi(x)\,d\sigma(x)
	\end{equation*}
	where $\nu_x$ denotes the unit normal to $\partial K$ at $x$.
\end{lemma}

\begin{proof}
	The proof is a straightforward computation using integration by parts. Recall that via \Cref{def:convex-influence}, we have \rnote{Starting from the third equation below I didn't understand the rest of the proof but I'm sure you can convince me that it is okay} 
\begin{align}
	\TInf[K] &= \Ex_{\bx\sim N(0, I_n)}\sbra{K(\bx)\pbra{n- \|\bx\|^2}} \nonumber \\
	&= \int_K (n - \|x\|^2)\cdot\phi(x)\,dx \nonumber\\
	&= \int_K \calL\pbra{\frac{\|x\|^2}{2}}\cdot\phi(x)\,dx  \nonumber\\
	\intertext{where for a function $f:\R^n\to\R$ we define $\calL(f) := \Delta f - \abra{\nabla f, \nabla({\|x\|^2}/{2})}$. Integrating by parts then gives}
	\TInf[K] &= \int_{\partial K} \abra{x, \nu_x} \cdot \phi(x)\,d\sigma(x),\nonumber
\end{align}
completing the proof.
\end{proof}

\begin{remark}
	We note that the surface integral formulation of total convex influence can be viewed as analogous to the fact that the total influence of a Boolean function is equal to its average sensitivity (cf. Chapter 2 of~\cite{odonnell-book}). Although we will not require it for our purposes, we note that a similar formulation holds for the convex influence of a direction $v\in \S^{n-1}$ on $K$:
	\begin{equation*} \label{eq:neeman}
		\Inf_v[K] = \int_{\partial K} \abra{x, v}\cdot\abra{\nu_x, v}\cdot\phi(x)\,d\sigma(x)
	\end{equation*}
	where as before $\nu_x$ denotes the unit normal to $\partial K$ at $x$.
\end{remark}

\subsection{Bounds on the Convex Influence of Polytopes}
\label{sec:influence-structural-analogs}

%In this section, we obtain bounds on the convex influence of polytopes which suggest an analogy between Boolean CNF formulas and intersections of halfspaces which may be of independent interest. \Cref{prop:convex-boppana} will later be used in \Cref{subsec:convex-influence-lower-bound} to lower bound the number of facets needed to $0.001$-approximate the $\ell_2$ ball of volume $1/2$; \Cref{prop:influence-width-ub,prop:size-to-width} will not directly be linked to polytope approximation, and so we defer their proofs to \Cref{appendix:polytope-influence-bounds}.

In this subsection we give an upper bound on the total convex influence of an intersection of halfspaces in terms of the number of halfspaces. An analogous statement for CNF formulas over $\zo^n$, {showing that the influence of any $s$-clause CNF is at most $O(\log s)$,} was first given by Boppana~\cite{Boppana1997} using the technique of random restrictions~\cite{Hastad:86}. \footnote{In fact, Boppana~\cite{Boppana1997} obtains an upper bound of $O(\log^{d-1}(s))$ on the total influence of functions computed by depth-$d$ size-$s$ circuits.} The proof of \Cref{prop:convex-boppana} is inspired by the proof of \Cref{thm:nazarov} due to Nazarov; we give a self-contained proof of \Cref{prop:convex-boppana} below (see~\cite{ball-lecture} for a proof sketch of Nazarov's bound).

\begin{proposition}[Convex influence upper bound for intersections of halfspaces.]
%H\aa stad--Boppana analogues
\label{prop:convex-boppana}
	Let $K \sse\R^n$ be an intersection of $s>1$ halfspaces \red{that contains the origin}.\rnote{I don't want to be claiming anything about influence of convex sets that don't contain the origin} Then 
	\[\TInf[K] < 7\ln s.\]
\end{proposition}

We remark that the upper bound of \Cref{prop:convex-boppana} is best possible up to the hidden constant; the $\ell_\infty$ ball $K=\{x \in \R^n \ : \ \|x\|_\infty \leq r\}$ is an intersection of $2n$ halfspaces, and it is shown in Example~18 of \cite{DNS22} that for a suitable choice of $r$ we have $\TInf[K] = \Theta(\log n).$

\medskip

\begin{proof}[Proof of~\Cref{prop:convex-boppana}]
We let $K = \bigcap_{i=1}^s H_i$ for $s > 1$ where each $H_i$ is a halfspace of the form
	\[H_i := \cbra{x\in\R^n : \abra{x,v_i} \leq \theta_i}\]
	where $v_i \in \S^{n-1}$ for $i\in[s]$.  \red{Note that each $\theta_i \geq 0$ since $K$ contains the origin.}
	Using \Cref{lem:neeman}, we have \rnote{The red $\red{\partial H_i \cap \partial K}$ was $\partial(H_i\cap K)$, but since $K$ is contained in $H_i$ we have $H_i \cap K = K$ and so $\partial (H_i \cap K)$ is just $\partial K$, right? I had to change a few things further down too because of this, the changed things are in red.}
	\begin{align}
		\TInf[K] &= \int_{\partial K} \abra{x,\nu_x}\cdot\phi(x)\,d\sigma(x) \nonumber\\
		&= \sum_{i=1}^s \pbra{\int_{\red{\partial H_i \cap \partial K}} \abra{x,\nu_x}\cdot\phi(x)\,d\sigma(x)} \label{eq:useful}.
	\end{align}
	\red{Now, we observe that (i) $\GSA(K) = \sum_{i=1}^s \pbra{\int_{\red{\partial H_i \cap \partial K}} \phi(x)\,d\sigma(x)}$; (ii) for $x \in \partial H_i \cap \partial K$ we have $\abra{x,\nu_x}=\theta_i$; and (iii) for each $i \in [s]$, we have $\int_{\partial H_i \cap \partial K} \phi(x)\,d\sigma(x) \leq \int_{\partial H_i } \phi(x)\,d\sigma(x)=\GSA(H_i)$.  Combining these three observations, we get that}
	\begin{align}
(\ref{eq:useful})		&\red{\leq \max_{i \in [s]:\theta_i\leq \sqrt{2 \ln s}} \theta(i) \cdot \GSA(K) + \sum_{\substack{j \in [s] \\ \theta_j > \sqrt{2\ln s}}} \theta_j\cdot\GSA(H_j).} 
		\label{eq:bop-sum}
	\end{align}
	We will control each of the two quantities in \Cref{eq:bop-sum} separately. For the first, we have that 
	\begin{equation} \label{eq:bop-sum-1}
\max_{i \in [s]:\theta_i\leq \sqrt{2 \ln s}} \theta(i) \cdot \GSA(K)  \leq \sqrt{2\ln s}
\pbra{\sqrt{2 \ln s} + 2}< 5\ln s,
	\end{equation}
	where the first inequality is by Nazarov's bound on GSA (\Cref{thm:nazarov}). For the second sum, we have that
	\begin{align}
		\sum_{\substack{j \in [s] \\ \theta_j > \sqrt{2\ln s}}} \theta_j\cdot\GSA(H_j) 
		&= \sum_{\substack{j \in [s] \\ \theta_j > \sqrt{2\ln s}}} \theta_j \cdot e^{-\theta_j^2/2}\nonumber\\
		& \leq s\cdot\max_{j : \theta_i > \sqrt{2\ln s}} \cbra{\theta_j\cdot e^{-\theta_j^2/2}}. \label{eq:gaga} 
		\end{align}
Since $xe^{-x^2/2}$ is a decreasing function for $x\geq 1$, and since $s >1$, it follows that $\theta_j\cdot e^{-\theta_j^2/2}$ is maximized for $\theta_j = \sqrt{2\ln s}$ which lets us conclude that
\begin{align}
(\ref{eq:gaga}) \leq \sqrt{2 \ln s} < 2 \ln s.\label{eq:bop-sum-2}
	\end{align}
	The result follows from \Cref{eq:bop-sum,eq:bop-sum-1,eq:gaga,eq:bop-sum-2}.
\end{proof}

\subsubsection{Digression} 
\label{sec:digression}
We briefly digress to continue exploring the analogy between intersections of halfspaces over $\R^n$ and CNF formulas over the Boolean hypercube. In addition to the size of a CNF, another natural complexity measure associated to a CNF is the \emph{width} of the CNF, which is the maximum number of literals in any clause of the CNF. The following proposition is analogous to the well-known fact that the total influence of a CNF of width $w$ is at most $O(w)$ (cf. Proposition 4.7 of~\cite{odonnell-book}; see~\cite{Amano-dnf} for the sharp constant). 

\begin{proposition} \label{prop:influence-width-ub}
	For $w>0$, let $K\sse\R^n$ be an intersection of $s$ halfspaces of the form 
	\[
	K = \bigcap_{i=1}^s H_i 
	\qquad\text{where}\qquad 
	H_i := \{x\in\R^n : \abra{x,v_i} \leq w\}
	\]
	for unit vectors $v_i \in \S^{n-1}$, and furthermore suppose $0^n\in K$.  Then we have 
	\[\TInf[K] \leq O(w^2).\]
\end{proposition}

{It is folklore that any $s$-clause CNF over $\zo^n$ can be $\eps$-approximated by a CNF in which each clause contains at most $\log(s/\eps)$ literals.  The following proposition gives an analogous result for intersections of halfspaces:}
% also straightforward to show that intersections of a small number of halfspaces can be well-approximated by intersections of not-too-wide halfspaces as well:

\begin{proposition} \label{prop:size-to-width}
	Let $K\sse\R^n$ be an intersection of $s$ halfspaces. For any $\eps >0$, there exists a set $L \sse\R^n$ which is an intersection of at most $s$ halfspaces $\{H_i\}$ where each $H_i$ is of the form
	\[ H_i := \cbra{x\in\R^n : \abra{x,v_i} \leq w}, \qquad\text{where}~w^2 = O\pbra{\log\pbra{\frac{s}{\epsilon}}},\]
	which satisfies $\dG(K, L) \leq \eps$.
\end{proposition}

As \Cref{prop:influence-width-ub,prop:size-to-width} will not be used in the rest of this section, we defer their proofs to~\Cref{appendix:polytope-influence-bounds}.


\subsection{Lower Bounds for Approximating Convex Sets with Maximal Influence}
\label{subsec:convex-influence-lower-bound}

We finally establish the following lower bound on approximating symmetric convex sets with maximal convex influence.  \red{(The specific constants in the theorem below were chosen mostly for concreteness; other constants could have been used instead.)}

\begin{theorem} \label{thm:high-influence-lb}
	Suppose $K\sse\R^n$ is a symmetric convex set with \red{$\Vol(K) = 1/2 \pm o_n(1)$ and} $\TInf[K]  \geq 0.1\sqrt{n}$. Then any polytope that $0.005$-approximates $K$ must have at least
	$2^{0.01\sqrt{n}{\red{-1}}}~\text{halfspaces}.$
\end{theorem}

We will use the following simple lemma, which says that when approximating symmetric convex sets, we may assume without loss of generality that our approximator is symmetric.
\red{(In the proof of \Cref{thm:high-influence-lb} we will use the symmetry both of the set $K$ and of the approximators to ensure that their convex influences are non-negative~\cite{DNS21itcs,DNS22}.)}\rnote{Is this true?}


\begin{lemma} \label{lem:symmetric-approximators}
	Suppose $K\sse\R^n$ \red{is symmetric and}\rnote{Added this - we want it in the theorem statement, right?} has $\vol(K) = 1/2 \pm o_n(1)$. Let $\eps < \red{0.499}$. If there exist $s$ halfspaces $H_1, \ldots, H_s$ such that 
	\[\dG\pbra{K, \cap H_i} \leq \frac{\eps}{2},\]
	then there exist $s$ slabs $S_1, \ldots, S_s$ such that 
	\[\dG\pbra{K, \cap S_i} \leq \epsilon\]
	where a \emph{slab} is a set of the form $\{x\in\R^n : |\abra{x, v}| \leq \theta\}$ for some unit vector $v\in\S^{n-1}$ \red{(i.e.~a symmetric intersection of two halfspaces)}.
\end{lemma}

\begin{proof}
	Suppose each halfspace $H_i$ is of the form 
	\[H_i = \cbra{x\in\R^n : \abra{x, v^{(i)}} \leq \theta_i }\]
	where $v^{(i)} \in \S^{n-1}$. Note that $0^n$ belongs to $H_i$ for all $i$ because $K$ is symmetric and has volume $1/2 \pm o_n(1)$ \red{(if $0^n \notin H_i$ then $\dG(K,\cap H_i)$ would be at least $\Vol(K)/2>0.2495>\eps/2,$ contrary to our assumption on $\eps$)}.
	We define 
	\[H'_i := \cbra{x\in\R^n : -\abra{x, v^{(i)}} \leq \theta_i } \qquad \text{and} \qquad S_i := H'_i \cap H_i.\]
	Note that each $S_i$ is a slab. 
%	We define the slabs $S_i$ by symmetrizing the halfspaces $H_i$, i.e. 
%	\[S_i := \cbra{x\in\R^n : \abs{\abra{x, v^{(i)}}} \leq \theta_i  }.\]
	Since $K$ is symmetric, we have 
	\[\dG(K, \cap H_i) = \dG(K, \cap H'_i) \leq \frac{\eps}{2}.\]
Since we have
	\[\dG(K, \cap S_i) \leq \dG(K, \cap H_i) + \dG(K, \cap H_i') \leq \epsilon,\]
	the proof is complete.
\end{proof}

We now turn to the proof of~\Cref{thm:high-influence-lb}:\snote{I think we just require the target set $K$ to be symmetric, not the approximators. {\bf Rocco:}  I'm not really comfortable talking about the influence of the approximators unless we know they contain the origin - will we know this if they're not symmetric?}  

\begin{proof}
Let $L'$ be a polytope that $0.005$-approximates $K$.
\red{By \Cref{lem:symmetric-approximators} there is a symmetric polytope
$L$, i.e.~an intersection of slabs, which has at most twice as many facets as $L$ and which $0.01$-approximates $K$.}
It suffices to show the following:
	\begin{equation} \label{eq:inf-lb-goal}
		\text{If}~\dG(L,K) < 6.25\times 10^{-7},~\text{then}~\TInf[L] \geq 7 \cdot 2.5\times 10^{-4} \cdot \sqrt{n}.
	\end{equation}
	Indeed, with \Cref{eq:inf-lb-goal} in hand, it follows that if $L$ has $2^{0.01 \sqrt{n}}$ halfspaces, then by \Cref{prop:convex-boppana} we have
	\[\TInf[L] < 7 \cdot 0.01 \cdot \ln(2) \sqrt{n}\] 
	which contradicts~\Cref{eq:inf-lb-goal} for a sufficiently small constant $c_1$. 
	
	\Cref{eq:inf-lb-goal} can be inferred along the lines of the proof of Theorem~A.1 from~\cite{o2007approximation}, but we give a slightly simpler argument below.
	% for the reader's convenience. 
	Our proof will make use of the Hermite basis; we refer the reader to~\Cref{appendix:hermite} for a primer on Hermite analysis over the Gaussian measure. 
	Writing $e_i \in \R^n$ for the standard basis vector along the $i^\text{th}$ coordinate direction, we have that 
	\[\Inf_{e_i}[K] = \sqrt{2}\cdot\wt{K}(2e_i).\]
		(This is an immediate consequence of the fact that the degree-2 univariate Hermite polynomial $h_2(x)$ is ${\pbra{1 - x^2} /{\sqrt{2}}}.$)
	Let $\alpha(K)$ be the vector of the convex influences of $K$ along the $n$ coordinate directions scaled by a factor of $1/\sqrt{2}$, i.e. 
	\[\alpha(K) := \pbra{\wt{K}(2e_1), \ldots, \wt{K}(2e_n)}\]
	with $\alpha(L)$ defined similarly. 
	
\begin{claim} \label{claim:anindya-paley-zyg}
	Suppose $K$ is as in the statement of~\Cref{thm:high-influence-lb}. Then at least $0.002$-fraction of directions $\{e_1, \ldots, e_n\}$ have 
	\[\Inf_{e_i}[K] \geq \frac{0.05}{\sqrt{n}}.\]
\end{claim}

\begin{proof}
	Let $\bi \sim [n]$ uniformly at random. We have 
	\[\Ex_{\bi \sim [n]}[\Inf_{e_{\bi}}[K]] \geq \frac{0.1}{\sqrt{n}}\qquad\text{and}\qquad \Varx_{\bi \sim [n]}\sbra{\Inf_{e_{\bi}}[K]} \leq \frac{1}{n}\]
	where the upper bound on the variance follows from Parseval's formula. Recall Cantelli's inequality, which says that for a non-negative random variable $\bX$ with mean $\mu$ and variance $\sigma$, 
	\[\Pr\sbra{\bX > \mu-\theta\sigma} \geq \frac{\theta^2}{1+\theta^2} \]
	for $\theta \in [0,1]$. Cantelli's inequality is a straightforward consequence of the Paley--Zygmund inequality. Since $\Inf_{e_{\bi}}[K]$ is non-negative due to the symmetry of $K$ (Proposition~9 of~\cite{DNS22}),
	it follows that 
	\[\Prx_{\bi\sim [n]}\sbra{\Inf_{e_{\bi}}[K] > \frac{0.05}{\sqrt{n}}} \geq \frac{0.0025}{1.0025} > 0.002,\]
	which completes the proof.
\end{proof}

Without loss of generality, let $\{e_1, \ldots, e_t\}$ be the coordinate directions for which $\Inf_{e_i}[K] \geq 0.05/\sqrt{n}$ where $t\geq 0.002n$, as guaranteed by~\Cref{claim:anindya-paley-zyg}. Suppose, now, for the sake of contradiction, that $\TInf[L] \leq 0.25\times 0.05\times 0.002 = 0.25\times 10^{-3}\sqrt{n}$. It then follows that at most $t/2$ of $\{e_1, \ldots, e_t\}$ have 
\[\Inf_{e_i}[L] \geq \frac{0.05}{2\sqrt{n}}.\]
(To see this, note that if this were not the case, then $\TInf[L] \geq 0.25 \times 10^{-3}\sqrt{n}$.) In other words, we have that for at least $t/2$ of the coordinates in $\{e_1, \ldots, e_t\}$, we have 
\[\Inf_{e_i}[L] \leq \frac{0.05}{2\sqrt{n}}.\]
Call these coordinates ``bad'' coordinates. It follows by Parseval's formula that 
\begin{align*}
\dist(K,L) &= \Ex_{\bx\sim N(0,I_n)}\sbra{(K(\bx) - L(\bx))^2} \\
&= \sum_{\alpha\in\N^n} (\wt{K}(\alpha) - \wt{L}(\alpha))^2 \\
&\geq \sum_{e_i~\text{is bad}} (\wt{K}(2e_i) - \wt{L}(2e_i))^2 \\
&\geq \frac{1}{2}\cdot\frac{0.0025\times 0.002}{4},	
\end{align*}
which is a contradiction.
\end{proof}

As a consequence of \Cref{thm:high-influence-lb}, we immediately obtain lower bounds for approximating the $\ell_2$ and $\ell_1$ balls of Gaussian measure $\approx 1/2$:
\snote{The $6.25\times 10^{-7}$ is a bit embarrassing, but hopefully it's okay? Do we want to leave a remark or something saying that we can wiggle constants appropriately?}

% as well as for Nazarov's body~\cite{Nazarov:03}:

\begin{example}[$\ell_2$ ball] \label{eg:ball-conv-inf}
	Example~13 of~\cite{DNS22} establishes that 
\[\TInf[B_2] = \Theta(\sqrt{n}).\]
\Cref{lem:neeman} and Gaussian isoperimetry, however, allow us to obtain a lower bound on the constant hidden by the $\Theta(\cdot)$: Since $B_2$ is an intersection of infinitely many halfspaces at distance $\sqrt{n}$ from the origin, we have 
\[\TInf[B_2] \geq \sqrt{n}\cdot\GSA(B_2) \geq \sqrt{n} \geq \sqrt{\frac{n}{2\pi}} \geq 0.398\sqrt{n}.\]
Together with~\Cref{thm:high-influence-lb}, this immediately implies that any $6.25\times 10^{-7}$-approximation to $B(\sqrt{n})$ requires {$2^{\Omega(\sqrt{n})}$} facets. This in turn implies that \Cref{thm:de-nazarov} is tight up to constant factors when $\eps = 6.25\times 10^{-7}$. 
\end{example}

\begin{examples}[Cross-polytope] \label{eg:cross-polytope-inf}
	Let $B_1$ be the cross-polytope, i.e. the set
	\[B_1 := \cbra{x\in\R^n : \|x\|_1 \leq\sqrt{\frac{2}{\pi}}n}.\]
	Note that $B_1$ is an intersection of $2^n$ halfspaces, and recall  from~\Cref{subsec:cramer-bounds} that $\vol(B_1) = 1/2 \pm o_n(1)$. 
	By the Gaussian isoperimetric inequality, we have that $\GSA(B_1) \geq 0.398$, and so using \Cref{lem:neeman} we have
	\[\TInf[B_1] = \sqrt{\frac{2}{\pi}n}\cdot\GSA(B_1) \geq 0.1\sqrt{n}.\]
	Together with~\Cref{thm:high-influence-lb}, this immediately implies that any $6.25\times 10^{-7}$-approximation to $B_1$ requires {$2^{\Omega(\sqrt{n})}$} facets. (Recall from~\Cref{thm:ell-p-approx} that $B_1$ can be $0.01$-approximated using $2^{\Theta(n^{3/4})}$ halfspaces.)
\end{examples}

%%%%%
%%%%%\begin{example}[Nazarov's body] \label{eg:naz-conv-inf}
%%%%%	Nazarov~\cite{Nazarov:03} established (via a probabilistic argument) the existence of a polytope $K$ with $2^{\Theta(\sqrt{n})}$ facets, each at Euclidean distance $\red{\Theta}(n^{1/4})$ from the origin, with $\GSA(K)  \geq 0.28 n^{1/4}$. It follows from \Cref{lem:neeman} that
%%%%%	\[\TInf[K] = \Theta(n^{1/4}) \cdot \GSA(K) = \Theta(\sqrt{n}).\]
%%%%%	\Cref{thm:high-influence-lb} thus implies that Nazarov's body cannot be approximated to constant accuracy by any polytope with $2^{o(\sqrt{n})}$ facets.
%%%%%\end{example}
%%%%%
%%%%%









==> sections/cross-polytope-and-friends-safe.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Improved Approximations for $\ell_p$ Balls for \red{$p\in[1,2]$}}
\label{sec:ell-p}

The main result of this section is a proof of the existence of approximators for the volume-$1/2$ $\ell_p$ balls, with $1 \leq p < 2$, that have a sub-exponential number of facets:

\begin{theorem} \label{thm:ell-p-approx}
For $1 \leq p < 2$, let $B_p$ denote the origin-centered $\ell_p$-ball in $\R^n$ that has $\Vol(B_p)=1/2.$  
Let $0<\eps<1$. Then for $1 \leq p < 2$, there exists a polytope $K_p$ which is the intersection of 
	\[ s = \exp\pbra{\text{\red{FILL-ME-IN}}}~\text{halfspaces}\]
	such that 
	$\dG(B, K_p) \leq \eps.$

(In the special case of $p=1$, we have a slightly improved bound of \[
s=\exp\pbra{\Theta\pbra{\pbra{\frac{\log(1/\epsilon)}{\epsilon}}^{3/2} n^{3/4}}}~\text{halfspaces.)}\]
\end{theorem}

In \Cref{subsec:cramer-bounds} we recall some \Cramer-type tail bounds on sums of  random variables which we will use; the key property of these bounds which we will exploit is that they give tight \emph{multiplicative} control on the relevant tails.
\Cref{subsec:ell-1-warmup} proves the $p=1$ ``special case,'' and introduces many of the main ideas for the general case.  Finally we prove the $1<p<2$ case in \Cref{subsec:ell-p-balls}.

\subsection{\Cramer-Type Large Deviations Bounds}
\label{subsec:cramer-bounds}

Roughly speaking, ``\Cramer-type'' tail bounds are results which state that under suitable conditions, a sum $\bS$ of random variables for which $\E[\bS]=0$ and $\Var[\bS]=1$ will have tail probabilities $\Pr[\bS \geq x]$ which are \emph{multiplicatively} close to the corresponding Gaussian tail bound $\Pr_{\bg \sim N(0,1)}[\bg \geq x].$
The most standard results of this type are for sums of \emph{independent} random variables, as in the following theorem:

\bigskip

\snote{TODO: Move Petrov's bound here.}

\bigskip

We will also require a \Cramer-type bound, due to \cite{hu2007cramer}, for when the sum is a sum of randomly chosen values that are drawn \emph{without} replacement from a finite population. In more detail, let $\bX_1,\ldots,\bX_\newN$ \rnote{Changed ``$N$'' to a macro, backslash-newN; it's $m$ now but we can make it whatever} be a random sample drawn without replacement from a finite population $\{a_1, \ldots, a_n\}$ with \rnote{What's ``$\red{(a^+_i)}$'' --- can we just replace this with $a_i$?}
\[\sumi a_i = 0 \qquad\text{and}\qquad \sumi \red{(a^+_i)}^2 = n,\]
 where $\newN < n$.  We \gray{will write $\mu := \Ex\sbra{\bX_1}$ and $\sigma^2 = \Varx\sbra{\bX_1}$,\rnote{Under the assumptions from the previous line of centered math, don't we just have $\mu=0,\sigma^2=1$ --- if so then let's get rid of the gray stuff in this sentence? I'll simplify the statement of the theorem based on this} and} will write \rnote{Made $S_\newN$ bold - this is in line with our usual convention, right?}
\[\bS_\newN := \sum_{i=1}^\newN \bX_i, \quad p := \frac{\newN}{n}, \quad q := 1-p, \quad\text{and}\quad \omega_n^2 := npq.\]

\begin{theorem}[Theorem~1.2 of~\cite{hu2007cramer}] \label{thm:hrw}
	There exists an absolute constant $A > 0$ such that 
	\rnote{Next line was
	\[\Prx_{}\sbra{\bS_\newN - \newN\mu \geq t\sigma\omega_n} = \pbra{1 - \Phi(x)}\pbra{1 + O(1)(1+t)^3\frac{\beta_{3n}}{\omega_n}}\]
	}
	\[\Prx_{}\sbra{\bS_\newN  \geq t\omega_n} = \pbra{1 - \Phi(x)}\pbra{1 + O(1)(1+t)^3\frac{\beta_{3n}}{\omega_n}}\]
	for \rnote{Was $0\leq t \leq \red{{\frac 1 A} \cdot} \min\cbra{\frac{\omega_n\sigma}{\max_k |a_k - \mu|}, \pbra{\frac{\omega_n}{\beta_{3n}}}^{1/3}}$} \red{$0\leq t \leq \red{{\frac 1 A} \cdot} \min\cbra{\frac{\omega_n}{\max_k |a_k|}, \pbra{\frac{\omega_n}{\beta_{3n}}}^{1/3}}$}, where
	\rnote{Was $\beta_{3n} := \sigma^{-3}\Ex\sbra{|\bX_1 - \mu|^3}$} \red{$\beta_{3n} := \Ex\sbra{|\bX_1|^3}$}.
\end{theorem}


\subsection{Warmup: Approximating the Cross-Polytope}
\label{subsec:ell-1-warmup}

In this subsection we first show that $2^{\Theta(n^{3/4})}$ halfspaces suffice to approximate the \emph{cross-polytope} $\CP$, which is the  $\ell_1$-ball of Gaussian volume $1/2$, to constant error. This introduces many of the ideas used in the proof of~\Cref{thm:ell-p-approx}, while keeping technicalities to a minimum.  

Recall that for $\bx\sim N(0,I_n)$ we have 
\begin{equation}
\label{eq:mean-var-ell1}
\Ex\sbra{\|\bx\|_1} = \sumi  \Ex\sbra{|\bx_i|} = \sqrt{\frac{2}{\pi}}n \quad\text{and}\quad \Varx[\|\bx\|_1] = \sumi \Varx\sbra{|\bx_i|} = \pbra{1-\frac{2}{\pi}}n.
\end{equation}
Writing $B_1 \sse\R^n$ for the convex set 
\[B_1 := \cbra{x\in\R^n : \|x\|_1\leq \sqrt{\frac{2}{\pi}}n},\]
it follows by the Berry--Esseen theorem~\cite{berry,esseen} (or alternatively, see Chapter~11 of~\cite{odonnell-book}) that $\Vol(B_1) = \red{1/2} \pm o_n(1)$. 
%As a warmup towards~\Cref{thm:ell-p}, we show that $2^{\Theta_{}(n^{3/4})}$ halfspaces suffice to approximate $B_1$:

\begin{theorem} \label{thm:ell-1-approx}
	Let $\Theta(1/\sqrt{n}) < \eps < 1$. There exists a set $L$ which is an intersection of 
	\[ s:= \exp\pbra{\wt{\Theta}\pbra{\frac{n^{3/4}}{\eps^{3/2}}}}~\text{halfspaces}\]
	such that $\dG(B_1, L) \leq O(\eps)$, where the $\wt{\Theta}$ hides $O(\log(1/\eps))$ factors. 
\end{theorem}

As in the proof of \Cref{thm:de-nazarov}, our construction is probabilistic. We start by defining our distribution over convex sets:

\begin{definition} \label{def:ell-1-naz}
	For $M, \newN, \theta > 0$, we write $\CP(M,\newN, \theta)$ to be the distribution over polytopes in $\R^n$ where a draw from $\CP(M,\newN,\theta)$ is obtained as follows:
	\begin{enumerate}
		\item Draw $M$ $\newN$-tuples from $[n]$ without replacement, i.e. draw 
		\[
%		\overline{\bi}^{(j)} := 
		\pbra{\i{j}_1, \ldots, \i{j}_\newN} \in {[n] \choose \newN} \quad\text{for}~1\leq j\leq M.\]
		\item For $j\in[M]$, define the convex set 
		\[\bC_j := \cbra{x\in\R^n : \sum_{k=1}^\newN |x_{\i{j}_{k}}| \leq \theta}.\]
		\item Output the convex set
		\[\bL := \bigcap_{j=1}^M \bC_j.\]
	\end{enumerate}
\end{definition}

Note that $\bC_j$ is the $\theta$-dilate of the unit $\ell_1$ ball in the $\newN$-dimensional subspace spanned by the vectors $\{e_{\i{j}_1},\ldots, e_{\i{j}_\newN}\}$ where $e_i$ denotes the standard $i^{\text{th}}$ basis vector.   

\begin{proofof}{\Cref{thm:ell-1-approx}}

We will establish~\Cref{thm:ell-1-approx} by showing that there exists a set in the support of $\CP(M,\newN,\theta)$ with the desired properties. Since each $\bC_j$ is an intersection of $2^\newN$ halfspaces, it follows that every set $\bL$ in the support of $\CP(M, \newN, \theta)$ is an intersection of $M\cdot 2^\newN$ halfspaces. 

As in the proof of~\Cref{thm:de-nazarov}, the existence of such a set follows from 
\[\Ex_{\bL\sim\CP(M,\newN,\theta)}\sbra{\Prx_{\bx\sim N(0,I_n)}\sbra{\bL(\bx) \neq B_1(\bx)}} \leq O(\eps),\]
which, by commuting the order of integration, is equivalent to showing that 
\begin{equation} \label{eq:cp-goal-1}
	\Ex_{\bx\sim N(0,I_n)}\sbra{\Prx_{\bL\sim\CP(M,\newN,\theta)}\sbra{\bL(\bx) \neq B_1(\bx)}} \leq O(\eps).
\end{equation}

As in the earlier argument, \Cref{eq:cp-goal-1} allows us to analyze the error incurred by our approximator on an ``$x$-by-$x$ basis.'' We set parameters
\[\din := \sqrt{\frac{2}{\pi}}n - \eps\sqrt{n} \qquad\text\qquad \dout := \sqrt{\frac{2}{\pi}}n + \eps\sqrt{n}.\]
By the discussion above and the Berry--Esseen theorem\rnote{Do we want to mention the Berry-Esseen theorem in the preliminaries, or is it part of the zeitgeist at this point? A compromise would be to cite e.g. a Wikipedia page the first time we mention it.}, we have that for $\bx\sim N(0, I_n)$,
	\[\mathrm{d}_{\mathrm{Kol}}\pbra{ \|\bx\|_1, N\pbra{\sqrt{\frac{2}{\pi}}n, \pbra{1-\frac{2}{\pi}}n} } \leq O\pbra{\frac{1}{\sqrt{n}}}\]
where $\mathrm{d}_{\mathrm{Kol}}$ denotes the Kolmogorov or CDF distance. Consequently, for $\eps > \Theta(1/\sqrt{n})$, we have that 
\begin{equation} \label{eq:boundary-pts}
	\Prx_{\bx\sim N(0,I_n)}\sbra{\din < \|x\|_1 < \dout} \leq O(\eps).
\end{equation}
\red{Intuitively, we will ``give up'' on points $x$ with $\din < \|x\|_1 < \dout$, and in the rest of the argument our focus will be on achieving high accuracy on other points. Towards this end, the following definition will be useful:}

\begin{definition} \label{def:ell-1-good-bad}
We say that a point $x\in\R^n$ is \emph{good} if it satisfies all three of the following properties:
\begin{enumerate}
	\item \begin{equation} \label{eq:bad-condition}
	\|x\|_2^2 - \frac{\|x\|_1^2}{n} \in \sbra{n\pbra{1-\frac{2}{\pi}}(1 - {o_n(1)}), n\pbra{1-\frac{2}{\pi}}(1 + {o_n(1)})}; \nonumber
\end{equation}
	\item $\max_{i\in[n]}|x_i| = {\Theta(\sqrt{\log n})}$; and
	\item $n^{-1}\sumi |x_i|^3 = {\Theta(1)}$.
\end{enumerate}
If $x$ is not good we say that it is \emph{bad}.
\end{definition}

\begin{claim} \label{claim:good-prob}
We have $\Prx\sbra{\bx~\text{is bad}} = O(\eps)$ where $\bx\sim N(0,I_n)$.
\end{claim}

\begin{proof}
	We show that each of Items 1, 2, and 3 from~\Cref{def:ell-1-good-bad} hold with probability at least $1-O(\eps)$.	
	Recalling that $\|\bx\|_2^2\sim \chi^2(n)$ for $\bx\sim N(0,I_n)$, we immediately get from~\Cref{prop:chi-squared-tail} that with probability at least $1-\eps$, 
	\[\|\bx\|_2^2 \in \sbra{n \pm \Theta\pbra{\sqrt{n\ln\pbra{\frac{2}{\eps}}}} } \subseteq \sbra{n \pm \Theta\pbra{ \sqrt{n\ln n} } } \]
	where we use the fact that $\eps \geq \Theta(1/\sqrt{n})$. 
For the 1-norm, recalling \Cref{eq:mean-var-ell1} \red{and again using $\eps \geq \Theta(1/\sqrt{n})$},
	Chebyshev's inequality gives that with probability at least $1-\eps$, 
	\[
	\|\bx\|_1 \in \sbra{\sqrt{\frac{2}{\pi}}n \pm \sqrt{\pbra{1-\frac{2}{\pi}}\frac{n}{\eps}}} \red{\sse} \sbra{\sqrt{\frac{2}{\pi}}n \pm \sqrt{\pbra{1-\frac{2}{\pi}}}n^{\red{3/4}}}
	\]
\red{(a much sharper bound is possible, but we will not need it)}.	
	It is then immediate that with probability at least $1-2\eps$, 
	\begin{align*}
		\|\bx\|_2^2 - \frac{\|\bx\|_1^2}{n} &\in \sbra{n\pbra{1-\frac{2}{\pi}} \pm \Theta(\red{n^{3/4}})}\\
		&\sse \sbra{n\pbra{1-\frac{2}{\pi}}\left(1\pm o_n(1)\right)},
	\end{align*}
	proving Item~1. 
	
	\red{For Item~2, by a standard Gaussian tail bound (\Cref{prop:gaussian-tails}) we have that $\Pr\sbra{|\bx_i| > 2\sqrt{\ln n}} < 1/n^2$ for each $i \in [n],$ so a union bound over all $i \in [n]$ gives that $\Pr[\max_{i \in [n]} |\bx_i| \leq 2\sqrt{ \ln n}] > 1 - {\frac 1 n}$, which is at least $1 - \eps$ since $\eps >\Theta(1/\sqrt{n}).$}
	\rnote{I replaced the following with the red stuff since it seemed shorter and simpler (we don't need to introduce concentration of Lipschitz functions of Gaussian vectors):
	
		Item~2 is immediate from the concentration of Lipschitz functions of Gaussian vectors. In particular, note that $\|\cdot\|_{\infty}$ is $1$-Lipschitz, and so we have by Theorem~5.2.2 of~\cite{vershynin2018high} that
	\[\Prx_{\bx\sim N(0,I_n)}\sbra{\abs{\|\bx\|_{\infty} - \Ex_{\by\sim N(0,I_n)}\sbra{\|\by\|_{\infty}}} \geq t } \leq \exp\pbra{-\Theta\pbra{t^2}}.\]
	Recalling that $\E\sbra{\|\by\|_{\infty}} = \Theta\pbra{\sqrt{\log n}}$ (see for example Appendix~A of~\cite{chatterjee2014superconcentration}) and taking $t=\Theta\pbra{\sqrt{\ln(1/\epsilon}}$, we get that with probability at least $1-\eps$, 
	\[\|\bx\|_\infty \in \sbra{\Theta\pbra{\sqrt{\log n}} \pm \Theta\pbra{\sqrt{\log\pbra{\frac{1}{\eps}}}}}.\]
	Recalling that $\eps \geq \Theta(1/\sqrt{n})$, Item~2 follows. 
}

	Turning to Item~3, it is known~\cite{winkelbauer2012moments} that
	\[\Ex_{\bx\sim N(0, I_n)}\sbra{\sumi|\bx_i|^3} = \sqrt{\frac{8}{\pi}}n \qquad\text{and}\qquad \Varx_{\bx\sim N(0, I_n)}\sbra{\sumi |\bx_i|^3} \leq 25n.\]
	Consequently, by Chebyshev's inequality we have that with probability at least $1-\eps$ over $\bx\sim N(0,I_n)$, the following holds:
	\[
%	\sqrt{\frac{8}{\pi}} - \frac{5}{\sqrt{n}} \leq 
	\sqrt{\frac{8}{\pi}} - \frac{5}{\sqrt{\eps n}} \leq \frac{1}{n}\sumi |\bx_i|^3 \leq \sqrt{\frac{8}{\pi}} + \frac{5}{\sqrt{\eps n}}.
%	\leq \sqrt{\frac{8}{\pi}} + \Theta\pbra{\frac{1}{n^{1/4}}},
	\]
	Once again, recalling that $\eps \geq \Theta(1/\sqrt{n})$ immediately implies Item 3.
	\rnote{Super-minor stylistic nitpick: I removed ``for $n$ large enough'' --- if we're in a setting where we're using big-$\Theta$-of-$n$ type notation, we are already implicitly only talking about the large-enough-$n$ regime.}
\end{proof}


We will show that for an appropriate choice of parameters $M, \newN,$ and $\theta$, we have that whenever $\|x\|_1 \notin (\din,\dout)$ and $x$ is good,
\begin{equation} \label{eq:cp-goal-2}
	\Prx_{\bL\sim\CP(M, \newN, \theta)}\sbra{\bL(x)\neq B_1(x)} \leq O(\eps). 
\end{equation}
\Cref{eq:cp-goal-2,eq:boundary-pts}, together with~\Cref{claim:good-prob}, immediately imply~\Cref{eq:cp-goal-1}, which completes the proof of~\Cref{thm:ell-1-approx}. 

\paragraph{Case 1: $\|x\|_1\leq\din$ \red{and $x$ is good}.} In this case, note that $B_1(x) = 1$, and so it suffices to show that for any \red{fixed $j \in [M]$}, we have 
\begin{equation} \label{eq:ell-1-yes-goal}
	\Prx_{\CP(M,\newN,\theta)}\sbra{x \in \bC_j} \geq 1-\frac{\eps}{M},
\end{equation}
since this immediately implies that 
\[\Prx_{\CP(M,\newN,\theta)}\sbra{x \in \bigcap_{j=1}^M \bC_j} \geq \pbra{1-\frac{\eps}{M}}^M \geq 1-\eps,\]
as desired. Let $x^+$ denote the vector $(|x_1|, \ldots, |x_n|)$, \red{and observe that since $x$ is good, so is $x^+$.}
%Note that membership (or non-membership) of $x$ in $\bL$ is solely a function of $x^+$. 

We will make use of the \Cramer-type bound given by \Cref{thm:hrw} to prove~\Cref{eq:ell-1-yes-goal}. In order to apply \Cref{thm:hrw}, let \rnote{Minor: it seems a little notationally weird for $v^+$ to be a vector which has some negative entries; are we saving just ``$v$'' for something else?}
\[v^+ := x^+ - \frac{\|x\|_1(1, \ldots, 1)}{n} \qquad
\text{and so}
\qquad \sumi v^+ = 0. 
\]
Note that 
\[\sumi \pbra{v_i^+}^2 = \|x^+\|_2^2 - \frac{\|x^+\|_1^2}{n} \in \sbra{n\pbra{1-\frac{2}{\pi}}\pbra{1\pm {o_n(1)}}}\]
where the inclusion holds because $x^+$ is good (cf. Item~1 of~\Cref{def:ell-1-good-bad}). In particular, let $c_x$ be such that 
\[\sumi \pbra{v_i^+}^2 = c_xn, \quad\text{i.e.}\quad c_x = \pbra{1-\frac{2}{\pi}}\pbra{1\pm {o_n(1)}}.\]
%For $n$ sufficiently large, we have $c = \Theta\pbra{1 - 2/\pi}$; we assume this to be the case.\snote{We might actually have to carry around the multiplicative factor.}
For convenience, we define
\[c := 1 - \frac{2}{\pi}\]
and so $c_x = c(1\pm o_n(1))$. 

We will apply~\Cref{thm:hrw} to the finite population $\{a_i\}_{i\in[n]}$, where
\[a_i := \frac{v^+_{\red{i}}}{\sqrt{c_x}}.\]
It is immediate that $\sumi a_i = 0$ and that\rnote{Again let's replace the $\red{(a_i^+)}$ with just $a_i^2$?} $\sumi \red{(a_i^+)}^2 =n$, as required by~\Cref{thm:hrw}. Furthermore, we have
\rnote{I think it might not be ideal to just use $\omega_n^2 = \Theta(\newN)$, because then you will get into a situation where you have the big-theta in the $\blue{\Theta(t\sqrt{\newN})}$ in the equation below, and that makes things murkier later --- there's a mismatch with the green event further down.  (I like having something very explicit for the green thing, without any big-$\Theta$,  because I feel like it's best to give a very explicit expression for $\theta$ without any big-$\Theta$ notation in it. Note that in the current expression for $\theta$ we have some weirdness, which I marked in blue...

Maybe the best bet is to just carry around the $\omega_n$ for as long as possible, i.e. just replace the blue $\blue{\Theta(t \sqrt{\newN})}$ with $\omega_n$ and carry that around for as long as we can?  Let's chat about this...}
\[\omega_n^2 = \newN\pbra{1-\frac{\newN}{n}} = \Theta(\newN).\]
(The final equality holds because, looking ahead, we will have $\newN \red{\approx n^{3/4}}$.) Furthermore, since $x$ is good, by Item~2 of~\Cref{def:ell-1-good-bad} we have that $\max_k |a_k| = \Theta(\sqrt{\log n})$, and by Item~3 of ~\Cref{def:ell-1-good-bad} we have that $\beta_{3n} = \Theta(1)$. It follows from~\Cref{thm:hrw} that for any fixed $j \in [M],$ with $\bC_j$ as in~\Cref{def:ell-1-naz}, we have 
\[\Prx_{\CP(M,\newN,\theta)}\sbra{a_{\i{j}_1} + \ldots + a_{\i{j}_\newN}\geq \blue{\Theta(t\sqrt{\newN})}} = \pbra{1-\Phi(t)}\pbra{1 + \frac{O(1)(1+t)^3}{\sqrt{\newN}}}\]
for $t \leq O\pbra{\min\cbra{\sqrt{\newN/\log n}, \newN^{1/6}}} = O(\newN^{1/6})$.

Recalling that $a = c_x^{-1/2}\pbra{x^+_{\red{i}} - \frac{\|x\|_1}{n}}$, note that the event $a_{\i{j}_1} + \ldots + a_{\i{j}_\newN} \geq \green{t\sqrt{\newN}}$ is the same as the event 
\[\frac{1}{\sqrt{c_x}}\sum_{k=1}^\newN \pbra{x^+_{\i{j}_k} - \frac{\|x\|_1}{n}} \geq t\sqrt{\newN}, \qquad\text{or equivalently,}\qquad  \sum_{k=1}^\newN x_{\i{j}_k}^+ \geq \|x\|_1\frac{\newN}{n} + t\sqrt{c_x\newN}.\]
This motivates our choice of $\theta$ where we will take \red{$t = \Theta(\newN^{1/6})$} 
\rnote{Maybe we're better off here having ``$t = c_1 \newN^{1/6}$ for a sufficiently small absolute constant $c_1$''?} in the above, i.e. we set
\rnote{It's weird to have both big-Theta notation and the constant $\sqrt{c}$}
\[\theta:= \din\frac{\newN}{n} + \Theta\pbra{\newN^{1/6}}\sqrt{\newN c} = \sqrt{\frac{2}{\pi}}\newN - \frac{\eps \newN}{\sqrt{n}} + \blue{\Theta\pbra{\newN^{2/3}\sqrt{{c}}}}.\]

We will require the following monotonicity claim, which allows us to only worry about points with maximal $\ell_1$ norm. 

\begin{claim} \label{claim:monotonicity}
\rnote{At the start of this {\bf Case 1} we had that $x$ was the point with $\|x\|_1 \leq \din$; in this claim we're calling that $y$ and $x$ is a rescaling of it - this is a little confusing. Is it okay for me to rename variables? e.g. make the $y$ of this claim into $x$ and the $x$ of this claim into $z$?}
	Suppose $y \in \R^n$ with $\|y\|_1\leq \din$. Let $x = ty$ for $t \geq 1$ be such that $\|x\|_1 = \din$. Then
	\[\Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^n x^+_{\i{j}_k} \geq \theta } \geq \Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^n y^+_{\i{j}_k} \geq \theta }.\]
\end{claim}

This is immediate from the fact that the map 
\[y_{\i{j}_k} \mapsto t\cdot y_{\i{j}_k} = x_{\i{j}_k}\] 
gives a monotone coupling between the two random variables, and hence $x_{\i{j}_k}$ stochastically dominates $y_{\i{j}_k}$ (cf.~Theorem 4.2.3 of~\cite{roch-ch4}).

Using~\Cref{claim:monotonicity}, we have that for good $y$ with $\|y\|_1\leq\din$ and for $x$ as in~\Cref{claim:monotonicity}, 
\begin{align*}
	\Prx_{\CP(M,\newN,\theta)}\sbra{y \notin \bC_j} \leq \Prx_{\CP(M,\newN,\theta)}\sbra{x\notin \bC_j} &= \Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^\newN x^+_{\i{j}_k} \geq \theta} \\ 
	&=\Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^\newN a_{\i{j}_k} \geq \frac{\Theta(\newN^{1/6})\sqrt{\newN}}{1\pm o_n(1)} } \\
	&\stackrel{1\pm o_n(1)}{\approx} 1-\Phi\left(\Theta\pbra{\frac{\newN^{1/6}}{1\pm o_n(1)}}\right) \\
	&\leq \exp\pbra{-\Theta(\newN^{1/3})}.
\end{align*}
Note that the $(1\pm o_n(1))$ factor appears in the second term because $c_x = c(1\pm o_n(1))$.\snote{Rocco---does this seem okay to you?} This in turn motivates our choice of $M$, namely
\[M := \eps \cdot\exp\pbra{\Theta(\newN^{1/3})}.\]

As a consequence of this, we have that 
\[\Prx_{\CP(M,\newN,\theta)}\sbra{y\notin \bC_j} \leq \frac{\eps}{M},\]
as desired (cf.~\Cref{eq:ell-1-yes-goal}). 
	
\paragraph{Case 2: $\|x\|_1\geq\dout$ \red{and $x$ is good}.} In this case, we will show that for  
\ignore{a good $x$ and}any fixed $j\in[M]$, we have 
\begin{equation} \label{eq:ell-1-no-goal}
	\Prx_{\CP(M,\newN,\theta)}\sbra{x \in \bC_j } \leq 1 - \frac{\ln(1/\eps)}{M}.
\end{equation}
Indeed, if~\Cref{eq:ell-1-no-goal} holds, then we have that 
\[\Prx_{\CP(M,\newN,\theta)}\sbra{x \in \bigcap_{j=1}^M \bC_j} \leq \pbra{1 - \frac{\ln(1/\eps)}{M}}^M \leq \eps\]
as desired, completing the proof. {As in Case 1, an analogous statement to~\Cref{claim:monotonicity} holds, and hence we only have to establish~\Cref{eq:ell-1-no-goal} for $x$ with $\|x\|_1 =\dout$. In particular:}

\begin{claim} \label{claim:ell-1-dout-monotone}
	Suppose $y\in\R^n$ with $\|y\|_1\geq \dout$. Let $x = ty$ for some $t\leq 1$ be such that $\|x\|_1 = \dout$. Then 
	\[\Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^n y^+_{\i{j}_k} \geq \theta } \geq \Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^n x^+_{\i{j}_k} \geq \theta }.\]
\end{claim}

Writing $a_i$ as before, note that the event 
\[\sum_{k=1}^\newN a_{\i{j}_k} \geq t\sqrt{\newN} - \frac{2\newN\epsilon}{\sqrt{cn}}~~
\text{is the same as}~~\frac{1}{\sqrt{c_x}}\sum_{k=1}^\newN \pbra{x_{\i{j}_k} - \frac{\|x\|_1}{n} }\geq t\sqrt{\newN} -\frac{2\newN\epsilon}{\sqrt{cn}}.
\]
Note that this is equivalent to
\begin{equation} \label{eq:cowbell}
	\sum_{k=1}^\newN x_{\i{j}_k}^+ \geq \|x\|_1\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}}\sqrt{\frac{c_x}{c}} + t\sqrt{c_x\newN}.
\end{equation}
Recalling $\dout$, our choice of $\theta$, and the fact that $c_x = c(1\pm o_n(1))$, we can write
\begin{align}
	\theta &= \dout\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}} + \Theta(\newN^{2/3}\sqrt{c}) \nonumber \\
	&= \dout\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}}\sqrt{\frac{c_x}{c}} + \Theta(\newN^{2/3}\sqrt{c_x}) + \frac{2\newN\eps}{\sqrt{n}}\pbra{\sqrt{\frac{c_x}{c}} - 1} + \Theta(\newN^{2/3}\sqrt{c})\left(1 - \sqrt{1 \pm o_n(1)}\right) \nonumber \\
	&= \dout\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}}\sqrt{\frac{c_x}{c}} + \Theta(\newN^{2/3}\sqrt{c_x}) \pm o_n(1)\pbra{\frac{2\newN\eps}{\sqrt{n}} + \Theta(\newN^{2/3}\sqrt{c})} \nonumber \\ 
	&= \dout\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}}\sqrt{\frac{c_x}{c}} + \sqrt{c_x \newN}\cdot\pbra{\Theta(\newN^{1/6})(1 \pm o_n(1)) \pm o_n(1) \cdot 2\eps\sqrt{\frac{\newN}{nc_x}}} \nonumber\\
	&= \dout\frac{\newN}{n} - \frac{2\newN\eps}{\sqrt{n}}\sqrt{\frac{c_x}{c}} + \Theta\pbra{\newN^{1/6}(1 \pm o_n(1))}\sqrt{c_x \newN}. \label{eq:more-cowbell}
\end{align}
By~\Cref{claim:ell-1-dout-monotone}, we may assume that $\|x\|_1 = \dout$. This, together with~\Cref{eq:cowbell,eq:more-cowbell}, lets us write
\begin{align*}
	\Prx_{\CP(M,\newN,\theta)}\sbra{x\notin\bC_j} &= \Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^\newN x^+_{\i{j}_k} \geq \|x\|_1\frac{\newN}{n} - \frac{2\newN\eps }{n}\sqrt{\frac{c_x}{c}} + \Theta\pbra{\newN^{1/6}(1 \pm o_n(1))}\sqrt{c_x \newN} } \\ 
	&= \Prx_{\CP(M,\newN,\theta)}\sbra{\sum_{k=1}^\newN a_{\i{j}_k} \geq \pbra{\Theta\pbra{\newN^{1/6}(1 \pm o_n(1))} - 2\eps\sqrt{\frac{\newN}{cn}}}\sqrt{\newN}} \\
	&\stackrel{1\pm o_n(1)}{\approx} 1 - \Phi\pbra{\Theta\pbra{\newN^{1/6}(1 \pm o_n(1))} - 2\eps\sqrt{\frac{\newN}{cn}}} \\
	& \geq \exp\pbra{-\Theta\pbra{\newN^{1/6} - 2\eps\sqrt{\frac{\newN}{cn}}}^2} \\
	&\geq \frac{\epsilon}{M}\exp\pbra{\Theta\pbra{\frac{\eps \newN^{2/3}}{\sqrt{n}}}},
\end{align*}
where the multiplicative approximation is due to~\Cref{thm:hrw}, and the penultimate inequality is the standard tail bound $1-\Phi(x)\geq 0.25\exp(-x^2)$ for $x\geq 0$. 
Taking 
\[\newN := \Theta\pbra{\pbra{\frac{\ln(1/\eps) + \ln\ln(1/\eps)}{\eps}}^{3/2} n^{3/4}},\]
we get that 
\[\Prx_{\CP(M,\newN,\theta)}[x\notin \bC_j] \geq \frac{\ln(1/\eps)}{M},\]
establishing~\Cref{eq:ell-1-no-goal}.

Finally, note that the number of halfspaces in our approximator to $B_1$ is 
\[M\cdot 2^\newN = 
\red{\exp\pbra{\Theta\pbra{\pbra{\frac{\log(1/\epsilon)}{\epsilon}}^{3/2} n^{3/4}}}},\]
\rnote{I replaced 
\[
\exp\pbra{\Theta\pbra{\pbra{\frac{\log(1/\epsilon)+ \log\log(1/\eps)}{\epsilon}}^{3/2} n^{3/4}}}
\]
with the simpler-looking-and-asymptotically-the-same-(right?)
\[
\exp\pbra{\Theta\pbra{\pbra{\frac{\log(1/\epsilon)}{\epsilon}}^{3/2} n^{3/4}}}
\]
}
which completes the proof. 


	
	
\end{proofof}


%\begin{align*}
%	\Prx_{\CP(M,N,\theta)}\sbra{x\notin\bC_j} &= \Prx_{\CP(M,N,\theta)}\sbra{\sum_{k=1}^N x^+_{\i{j}_k} \geq \sqrt{\frac{2}{\pi}}N -\frac{\eps N}{\sqrt{n}} + \Theta(N^{2/3}\sqrt{c})} \\
%	&= \Prx_{\CP(M,N,\theta)}\sbra{\sum_{k=1}^N a_{\i{j}_{k}} \geq \pbra{N^{1/6} - 2\epsilon\sqrt{\frac{N}{cn}}}\sqrt{N}} \\
%	&\stackrel{1\pm o_n(1)}{\approx} 1-\Phi\pbra{n^{1/6} - 2\eps\sqrt{\frac{N}{cn}}} \\ 
%	&{\geq} \exp\pbra{-\Theta\pbra{N^{1/6} - 2\eps\sqrt{\frac{N}{cn}}}^2} \\
%	&\geq \frac{\epsilon}{M}\exp\pbra{\Theta\pbra{\frac{\eps N^{2/3}}{\sqrt{cn}}}},
%\end{align*}




















==> sections/dudley-proof.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Dudley's Convex Approximation Theorem}
\label{appendix:dudley}

We closely follow the exposition of Dudley's result by Har-Peled and Jones~\cite{har2019proof}.

\begin{proof}[Proof of~\Cref{thm:dudley}.]
	
\end{proof}






==> sections/generic-upper-bound.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Generic Bounds for Polytope Approximators}
\label{sec:generic-bounds}


\subsection{Upper Bounds}
\label{subsec:generic-ubs}

\begin{itemize}

\item 
\red{TODO: Here goes the Hausdorff-distance + Keith Ball combo.  We have been referring to this as ``naive Dudley''; it's the result which is obtained by integrating the $n^{1/4}$ generic GSA bound, and it gives us that any convex set can be $\eps$-approximated using something like $(n^{1/4}/\eps)^n$ many facets.  
}

\item \red{TODO:  The ``relative-error Dudley'' statement.  As of 6/27/2023, after fixing the bad geometric argument from earlier in June (when we erroneously assumed that the line from the origin to the surface was normal to the tangent hyperplane), it seems that this gives the following:  if $K$ has $\Vol(K) = 1-\delta$, then we can get an $\eps\delta$-approximator that has $\approx (n/\eps)^n$ many facets. Note that if e.g. $\delta = 2^{-n}$ and $\eps=0.001$ this is about $2^{n \log n}$ whereas naive Dudley would give $2^{n^2}$.  This improvement will be essential later for the $\ell_p$-ball approximation result, to achieve $2^{\sqrt{n} \log n}$.

(Note that the song and dance we do here does seem to be required for this relative-error result; it seems that spruced-up naive Dudley (replacing $n^{1/4}$ universal GSA bound by a sharper bound on GSA exploiting the fact that the volume is large) won't give a comparable result. See surface-area-of-large-volume-ball.heic photo; we computed there that for the volume-$(1-\eps)$ ball, the surface area is $\sqrt{\eps}$, so the naive Dudley argument using this would give $(\sqrt{\eps}/\eps)^n = (1/\eps)^{n/2}$ which is not good enough, it's $2^{n^2/2}$ at $\eps=1/2^n$.)}

\item \red{(Probably doesn't get mentioned in the paper) Anindya claims/observes that the statement we thought we had for most of June --- an \emph{absolute-error} Dudley improvement, giving $\tilde{O}(1/\eps)\cdot 2^{O(n)}$ facets for $\eps$-approximation of bodies that contain the ball --- probably isn't true.  He's right, and LSW +  our lower bound approach for Gaussian approximation based on that (see ``lower bounds for one-sided approximators (and maybe two-sided approximators?)'' email) rigorously establishes this. To recap it quickly:  our ``lower bounds for one-sided approximators (and maybe two-sided approximators?)'' email establishes that if you can $\eps=1/2^n$-approximate the volume-(1/2) ball w.r.t. Gaussian, then you can $\sqrt{n}/2^n$-approximate it w.r.t. Lebesgue/symmetric difference, but LSW establishes that such an approximator needs $2^{\Omega(n^2)}$ many facets.}

% We get bounds for both vertex and facet approximators.



\end{itemize}



\subsection{Lower Bounds}
\label{subsec:generic-lbs}

\subsubsection{VC Dimension Lower Bounds}
\label{subsec:vc-lbs}

Here goes the result from \cite{KOS:08} showing that there are $2^{2^{\Omega(\sqrt{n})}}$ many convex sets each pair of which are $1/44000$-far from each other.  Use this, plus VC dimension lower bounds, to infer the existence of a convex set which requires $2^{\Omega(\sqrt{n})}$ many vertices / facets to 0.01-approximate.

(I think this technology will not extend to give us a stronger facet/vertex lower bound for subconstant $\eps.$)


\subsubsection{Lower Bounds via Noise Sensitivity}
\label{subsec:gns-lbs}

\shivam{I guess here we can have the lower bound via the ``Baby switching lemma'' that we think we can prove using noise sensitivity + KOS08's hermite concentration + random zooms/OSTK's hyperconcentration?}


==> sections/lsw.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Lower Bounds Against High-Accuracy $\ell_2$ Ball Approximators}
\label{sec:lsw}

\red{Up for grabs later}


==> sections/noise-sensitivity-safe.tex <==
%!TEX root = ../polytope-approximation.tex

\newpage

\section{Average-case lower bounds via Gaussian noise sensitivity} \label{sec:noise-sensitivity}

The results of \Cref{sec:nonexplicit} show that there is some convex set $K \subset \R^n$ such that no  intersection of $2^{cn^{1/2}}$ many halfspaces can approximate $K$ to error better than $1/44000$. Since those results are non-constructive, though, they do not give us much information about what such a hard-to-approximate convex set ``looks like.''

In this section we describe a general structural property --- namely, having very high \emph{Gaussian noise sensitivity} (see \Cref{def:GNS}) at very low noise rates --- and show that for convex sets with this property, any intersection-of-halfspaces approximator must have $2^{n^{\Omega(1)}}$ halfspaces.  
\rnote{I think the statement of \Cref{thm:high-GNS-hard} is what we will be able to prove --- but it only makes sense to state this version of it if we are confident that there actually exist convex sets with $\GNS_{n^{-c_1}}(K) \geq {\frac 1 2} - n^{-c_2}$. 
\Cref{sec:existence} states that the Nazarov body satisfies some geometric conditions which would give us this GNS bound, but I'm not 100\% sure that the Nazarov body actually satisfies those geometric conditions; let's talk about this at some point?
}
\gray{Perhaps more interestingly, we prove a \emph{strong} inapproximability result, showing that it is impossible for such intersections of halfspaces to achieve even a particular $(1/2 + o_n(1))$ accuracy; i.e.~we establish a so-called \emph{average-case} lower bound.  More precisely, we prove the following:

\begin{theorem} \label{thm:high-GNS-hard}
Fix any constants $c_1,c_2>0$.
Let $K \subset \R^n$ be a convex set such that $\GNS_{n^{-c_1}}(K) \geq {\frac 1 2} - n^{-c_2}$.
Then there are constants $c_3,c_4$ (depending on $c_1,c_2$) such that for $L \subset \R^n$ any intersection of $\red{BLAH_2=2^{n^{c_3}}}$ many LTFs, we have
$\Vol(K \ \triangle \ L) \geq 1/2 - n^{-c_4}.$
\end{theorem}
}

(See \Cref{sec:existence} for the existence of convex sets $K$ with the claimed Gaussian noise sensitivity.)


\subsection{Random Zooms and Local Hyperconcentration}
\label{subsec:zoom-prelims}

\cite{OSTK21} introduced the notion of a ``random zoom'' of a function over Gaussian space and observed that it is a natural analogue of the well-studied notion of a random restriction of a function defined over the Boolean cube $\{-1,1\}^n$.  Random zooms are defined as follows:

\begin{definition}
    For a polynomial $p: \R^n \to \R$, $0 \leq \lambda \leq 1$, and $x \in \R^n$, we define the function $\zoom{p}{\lambda}{x}$ by
    \[
        \zoom{p}{\lambda}{x}(y) = p\pbra{\sqrt{1-\lambda} x + \sqrt{\lambda} y},
    \]
and we refer to the function $\zoom{p}{\lambda}{x}(\cdot)$ as the \emph{$\lambda$-zoom of $p$ at $x$}.
\end{definition}

For intuition, if $x \in \R^n$ is fixed we view $\sqrt{1-\lambda} x + \sqrt{\lambda} \by$ as a ``$\lambda$-noisy'' version of~$x$, and we view changing a function~$p$'s input from $\bx \sim N(0,I_n)$ to $\sqrt{1-\lambda} x + \sqrt{\lambda} \by$ as ``zooming into $p$ at~$x$ with scale~$\lambda$.''
We note that if $p$ is a degree-$d$ polynomial then so is $\zoom{p}{\lambda}{x}$, for any $\lambda<1$.
%\rnote{remove this sentence if we don't end up using it}

The following observation will be useful:
\begin{observation} \label{obs:completion-to-Gaussian}
If $\bx, \by \sim N(0,I_n)$ are independent and $0 \leq \lambda \leq 1$, then $\sqrt{1-\lambda} \bx + \sqrt{\lambda} \by$ is distributed identically to $\bz \sim N(0,I_n)$.  Thus the distribution of $\zoom{f}{\lambda}{\bx}(\by)$ is identical to $f(\bz),$ for any function $f$ and any $0 \leq \lambda \leq 1.$
\end{observation}

\Cref{obs:completion-to-Gaussian} is similar to how, in the Boolean function context of $f: \bn \to \R$, evaluating a random restriction on $f$ at a uniform random input is the same as evaluating $f$ at a uniform random input; see \cite{OSTK21} for a more detailed discussion of how random zooms for functions over Gaussian space are analogous to random restrictions of functions over $\bn$.

The ``Gaussian noise'' (or ``Ornstein--Uhlenbeck'') operator (see, e.g., \cite[Def.~11.12]{odonnell-book}) corresponds to the expectation of the zoom of a function:
\begin{definition} \label{def:gaussian-noise-operator}
    Given $0 < \rho \leq 1$, the operator $\U_\rho$ acts on polynomials $p : \R^n \to \R$ via
    \[
        (\U_\rho p)(x) = \Ex_{\by \sim N(0,I_n)}\sbra{p\pbra{\rho x + \sqrt{1-\rho^2} \by)}} = \Ex_{\by \sim N(0,I_n)}\sbra{ \zoom{p}{(1-\rho^2)}{x}(\by)}.
    \]
The operator $\U_\rho$ acts diagonally in the Hermite polynomial basis $(h_\alpha)_{\alpha \in \N^n}$:
    \begin{equation}    \label{eqn:U-formula}
        \U_\rho p = \sum_{\alpha \in \N^N} \rho^{|\alpha|} \wh{p}(\alpha) h_\alpha.
    \end{equation}
    In particular, if $p$ is a degree-$d$ polynomial, so too is $\U_\rho p$.

    Following \cite{OSTK21}, we will need to extend the definition of $\U_\rho$ to $\rho > 1$, which we can do via the formula \Cref{eqn:U-formula}; equivalently, by stipulating that $\U_{\rho^{-1}} = \U_{\rho}^{-1}$. Now we can define the \emph{hypervariance} of a function:
\end{definition}

\begin{definition} \label{def:hypervar}
    Let $g: \R^n \to \R$ be a polynomial.  For $R > 1$, we define the \emph{$R$-hypervariance} of~$g$ to be
    \[
        \HV_R[g] := \Var[\U_R g] = \sum_{\alpha \neq 0} R^{2|\alpha|} \wh{g}(\alpha)^2.
    \]
    (For $R = 1$, this reduces to the usual variance of~$g$.)
    If $\HV_R[g] \leq \eps \|g\|^2_2$, then we say that $g$ is \emph{$(R,\eps)$-attenuated}.
\end{definition}


The key structural result of \cite{OSTK21} states, roughly speaking, that a random zoom of a low-degree polynomial is very likely to be ``hyperconcentrated.'' In more detail, Theorem~85 of \cite{OSTK21}, specialized to the case that its ``nice'' distribution $(g_{\bup})_{\bup \sim \Upsilon}$ is a single degree-$d$ polynomial $p$, gives us the following:

\begin{theorem} [Local Hyperconcentration Theorem for a single polynomial, Theorem~85 of \cite{OSTK21}] \label{thm:OSTK-main-theorem}
There exists a constant $c>0$ so that for any $1>\eps,\beta>0$ and $R\geq 1$
\rnote{Daniel's statement of this theorem in his appendix said ``$R$ sufficiently small'', but from skimming his proof I don't think this is actually required, so I took it out.}, if $p(x_1,\dots,x_n)$ is a degree-$d$ polynomial, then taking
$$
\lambda \leq \frac{c\eps \beta}{R d^{9/2}},
$$
for $\bx \sim N(0,I_n)$ with probability at least $1-\beta$ we have that
$$
\hypvar_R(p_{\lambda|\bx}) \leq \eps^2  \| p_{\lambda|\bx}\|_2^2  
\quad
\text{(i.e.~$p_{\lambda|\bx}$ is $(R,\eps)$-attenuated).}
$$
\end{theorem}
We also recall the following result from \cite{OSTK21}, which roughly speaking says that ``attenuated polynomials are very likely to take values that are multiplicatively close to their means'':
\begin{proposition} [Proposition~32 of \cite{OSTK21}] \label{prop:atten-hyperconcy}
    Let $g$ be a polynomial that is $(R,\eps)$-attenuated, with $R \geq \sqrt{2}$ and $\eps \leq 1$. Write $\mu = \E[g]$ \red{and assume $\mu \neq 0$}.\rnote{With head hung in shame I have to say that \cite{OSTK21}'s Prop.~32 doesn't include the line ``and assume $\mu \neq 0$.'' But the statement is clearly false if $\mu=0$ --- by the definition of $\approx_{\gamma}$, if $\mu=0$ it would have to be the case that the Gaussian polynomial $g(\bx)$ takes value 0 at least, say, 0.1 of the time, which is preposterous. Proposition~25 of \cite{OSTK21}, which is used in its proof, implicitly assumes that $\mu$ is nonzero.}
Then for $0 < \gamma \leq 1$, for $\bz \sim N(0,I_n)$ we have $g(\bz) \approx_{\gamma} \mu$ (and hence $\sign(g(\bz))=\sign(\mu)$) except with probability at most $(2\sqrt{\eps}/\gamma)^{\frac12 R^2 + 1}$.
\end{proposition}

\subsection{PTFs and intersections of halfspaces collapse under random zooms}
\label{sec:collapse}

\Cref{thm:OSTK-main-theorem} and \Cref{prop:atten-hyperconcy} together give us that a random zoom of any degree-$d$ PTF will with high probability become a close-to-constant function:

\begin{corollary} [Random zooms of PTFs are close-to-constant whp]  \label{cor:zoom-close-to-constant}
Let $f: \R^n \to \{-1,1\}$, $f=\sign(p)$ be a degree-$d$ PTF, and let $0<\lambda<c'/d^{9/2}$ for a sufficiently small constant $c'$.  Then for any $0<\tau \leq 1$, we have
\begin{equation} \label{eq:bound}
\Prx_{\bx \sim N(0,I_n)}\sbra{\Var(\zoom{f}{\lambda}{\bx})\geq \tau} \leq 
{\frac {C d^{9/2} \lambda}{\tau}},
\end{equation}
where $C>0$ is a universal constant.
\end{corollary}

\begin{proof}
We assume that $p$ is a non-constant polynomial since otherwise the claim is trivially true.
Let $R=\sqrt{2}$, let $\eps=\tau/64$, and let $\lambda = c\eps \beta/(Rd^{9/2})$ where $c$ is the constant from \Cref{thm:OSTK-main-theorem}; equivalently, let $\beta$ be $16 \sqrt{2} d^{9/2} \lambda/(c\tau)$ (this is the RHS of \Cref{eq:bound}, taking $C = 16\sqrt{2}/c$). By taking $c'$ suitably small we have $\beta < 1$, and clearly $\eps<1$, so by \Cref{thm:OSTK-main-theorem} with probability at least $1-\beta$ over $\bx \sim N(0,I_n)$ we have that $\zoom{p}{\lambda}{\bx}$ is $(R,\eps)$-attenuated. 

Fix any outcome $x$ of $\bx$ such that $\zoom{p}{\lambda}{\bx}$ is $(R,\eps)$-attenuated and $\mu_{\bx} := \E[\zoom{p}{\lambda}{x}] \neq 0$ (note that the probability that $\mu_{\bx}=0$ is zero for $\bx \sim N(0,I_n)$, so the total probability of such $x$-outcomes is at least $1-\beta$). Taking $\gamma=1/2$ in \Cref{prop:atten-hyperconcy}, we get that $\zoom{f}{\lambda}{x}(\bz)$ equals $\sign(\E[\zoom{p}{\lambda}{x})$ except with probability at most $(2\sqrt{\eps}/\gamma)^{\frac12 R^2 + 1} = 16\eps=\tau/4$, and hence for such an $x$ we have $\Var(\zoom{f}{\lambda}{x}) \leq 4 \cdot {\frac \tau 4} \cdot (1-{\frac \tau 4}) \leq \tau.$
\end{proof}

To connect \Cref{cor:zoom-close-to-constant} with intersections of halfspaces, we recall the fact (from  \cite{KOS:08}) that any intersection of not-too-many halfspaces is close to a low-degree PTF:

\begin{theorem} [Low-degree PTF approximators for intersections of halfspaces, Theorems~15 and~20 of \cite{KOS:08}] \label{thm:KOS}
Let $K \subseteq \R^n$ be any convex set.  Then for any $\eps > 0$ there is a polynomial $p: \R^n \to \R$ of degree $d = O(\log(k)/\eps^2)$ such that the PTF $f=\sign(p)$ satisfies
\[
\Vol(K \ \triangle \ f^{-1}(1)) \leq \eps.
\]
\end{theorem}

Combining \Cref{thm:KOS} with \Cref{cor:zoom-close-to-constant}, we get that an intersection of few halfspaces simplifies to a close-to-constant function with high probability under a random zoom:

\begin{corollary} 
[Intersections of few halfspaces collapse to close-to-constant under random zooms]
\label{cor:polytope-collapse}
Let $L \subseteq \R^n$ be an intersection of at most $k$ halfspaces, and let $0<\delta<1.$
For a suitable choice of $\lambda = \Theta(\delta^{20}/(\log k)^{9/2}),$ we have
\[
\Prx_{\bx \sim N(0,I_n)} \sbra{\Var\pbra{\zoom{L}{\lambda}{\bx}} \geq \delta} \leq \delta.
\]
\end{corollary}

\begin{proof}
We argue by contradiction; so suppose that 
\begin{equation}
\label{eq:to-contradict}
\Prx_{\bx \sim N(0,I_n)} \sbra{\Var\pbra{\zoom{L}{\lambda}{\bx}} \geq \delta} > \delta.
\end{equation}
Let $\eps := \delta^2/64$.
By \Cref{thm:KOS}, there is a PTF $f=\sign(p)$ of degree $d := C_1 \log(k)/\eps^2$ which is an $\eps$-approximator for $L$, i.e. $\Vol(L \ \triangle \ f^{-1}(1)) \leq \eps.$
For a suitable choice of the hidden constant in $\lambda=\Theta(\delta^{20}/(\log k)^{9/2})$ (note that this choice of $\lambda$ satisfies the conditions of \Cref{cor:zoom-close-to-constant}) and $\tau=\sqrt{\eps}$, by \Cref{cor:zoom-close-to-constant} we have that 
\begin{equation} \label{eq:by-zoom-cor}
\Prx_{\bx \sim N(0,I_n)}\sbra{\Var(\zoom{f}{\lambda}{\bx})\geq \tau} \leq 
{\frac {C d^{9/2} \lambda}{\tau}} = \delta/2.
\end{equation}
Combining \Cref{eq:to-contradict} and \Cref{eq:by-zoom-cor}, we get that
\begin{equation} \label{eq:labor}
\Prx_{\bx \sim N(0,I_n)}
\sbra{
\Var\pbra{\zoom{L}{\lambda}{\bx}} \geq \delta
\text{~and~}
\Var(\zoom{f}{\lambda}{\bx})\leq \tau
} \geq \delta/2.
\end{equation}
Now, if $\Var_{\by}[a(\by)] \geq \delta$ and $\Var_{\by}[b(\by)] \leq \tau$ for $\{-1,1\}$-valued functions $a,b$ and $\delta>\tau$ then it must be the case that $\Pr_{\by}[a(\by) \neq b(\by)] \geq (\delta - \tau)/4.$
Recalling that $\delta=8\sqrt{\eps}$ and $\tau=\sqrt{\eps}$, \Cref{eq:labor} gives
\[
\Prx_{\bx \sim N(0,I_n)}\sbra{
\Prx_{\by \sim N(0,I_n)}\sbra{
\zoom{L}{\lambda}{\bx}(\by) \neq \zoom{f}{\lambda}{\bx}(\by)
} \geq 7\sqrt{\eps}/4
}\geq 4\sqrt{\eps},
\]
from which \Cref{obs:completion-to-Gaussian} gives 
\[
\Prx_{\bz \sim N(0,I_n)}\sbra{f(\bz) \neq L(\bz)} \geq
{\frac {7 \sqrt{\eps}} 4} \cdot {4 \sqrt{\eps}} = 7 \eps.
\]
This contradicts  $\Vol(L \ \triangle \ f^{-1}(1)) \leq \eps$, and the proof is complete.
\end{proof}

\subsection{Gaussian noise stability and expected variance after random zooms}

We recall the definitions of \emph{Gaussian noise stability} and \emph{Gaussian noise sensitivity}:

\begin{definition} [cf.~Definition~11.18 of \cite{odonnell-book}] \label{def:GNS}
For $f \in L^2(\R^n,\gamma)$ and $\rho \in [-1,1]$, the \emph{Gaussian noise stability of $f$ at $\rho$} is defined to be
\[
\Stab_\rho[f] = \Ex_{\bz,\bz'}\sbra{f(\bz)f(\bz')} = \abra{f,\U_{\rho}f},
\]
where $\bz,\bz'$ are $\rho$-correlated $N(0,I_n)$ Gaussians (equivalently, $\bz,\bg$ are independent $N(0,I_n)$ Gaussians and $\bz'=\rho \bz + \sqrt{1-\rho^2} \bg$).
For $\rho \in [0,1]$, the \emph{Gaussian noise sensitivity of $f$ at $\rho$} is
\[
\GNS_\rho[f] = {\frac 1 2} - {\frac 1 2} \Stab_{1-2\rho}[f].
\]
\end{definition}
We observe that for $f: \R^n \to \{-1,1\}$, we have
\[
\GNS_\rho[f] = \Prx_{\bz,\bz'}\sbra{f(\bz) \neq f(\bz')} = 2 \Prx_{\bz,\bz'}\sbra{f(\bz)=1, f(\bz') = -1},
\]
where now $\bz,\bz'$ are $(1-2\rho)$-correlated $N(0,I_n)$ Gaussians.

Gaussian noise sensitivity is important for us because the expected variance of $\zoom{K}{\lambda}{\bx}$, over $\bx \sim N(0,I_n)$, is exactly captured by Gaussian noise sensitivity:

\begin{lemma} \label{lem:expected-variance}
Let $K \subseteq \R^n$ be a convex set (viewed as a $\pm 1$-valued function on $\R^n$). For $0 \leq \lambda \leq 1$, we have that
\[
\Ex_{\bx \sim N(0,I_n)}
\sbra{
\Var_{\by \sim N(0,I_n)}[\zoom{K}{\lambda}{\bx}(\by)]
}
=
2\GNS_{\lambda/2}[K].
\]
\end{lemma}
\begin{proof}
Since $\Var[f(\by)]={\frac 1 2} \E_{\by,\by'}[(f(\by)-f(\by'))^2]$ where $\by,\by'$ are i.i.d., the LHS above is equal to
\begin{align*}
&
{\frac 1 2} \Ex_{\bx \sim N(0,I_n)}
\sbra{
\Ex_{\by,\by'\sim N(0,I_n)}\sbra{(\zoom{K}{\lambda}{\bx}(\by)-\zoom{K}{\lambda}{\bx}(\by'))^2}
}\\
&=
{\frac 1 2} \Ex_{\bx,\by,\by' \sim N(0,I_n)}
\sbra{
\pbra{K\pbra{\sqrt{1-\lambda} \bx + \sqrt{\lambda} \by} -
K\pbra{\sqrt{1-\lambda} \bx + \sqrt{\lambda} \by'}}^2
}\\
&= {\frac 1 2}
\Ex_{\bx,\by,\by' \sim N(0,I_n)}
\sbra{2 - 2
K\pbra{\sqrt{1-\lambda} \bx + \sqrt{\lambda} \by} 
K\pbra{\sqrt{1-\lambda} \bx + \sqrt{\lambda} \by'}
}\\
&= 1 - \Stab_{1-\lambda}[K] = 2 \GNS_{\lambda/2}[K]. \qedhere
\end{align*}
\end{proof}


\subsection{Proof of \Cref{thm:high-GNS-hard}:  Average-case lower bounds for convex sets that have high Gaussian noise sensitivity}

All the pieces are now in place for us to prove \Cref{thm:high-GNS-hard}. We first sketch the idea of the argument and then give quantitative details: Let $K$ be a convex set whose Gaussian noise stability at some low noise rate $\lambda/2$ is very high, i.e.~
$\GNS_{\lambda/2}(K) \geq {\frac 1 2} - o(1),$ and let $L$ be any intersection of ``not too many'' halfspaces. Our goal is to show that $L$ cannot be a good approximator for $K$; to do this, let us consider what happens if we apply a random zoom at noise rate $\lambda$ to both $K$ and $L$:

\begin{itemize}

\item  By the results of the previous subsection, the expected variance of $K$ after the random zoom is $2\GNS_\lambda[K]$, which is very close to 1; this means almost every outcome $\bx$ of the random zoom must be such that the convex body $\zoom{K}{\lambda}{\bx}$ has Gaussian volume very close to $1/2$.

\item But by the results of \Cref{sec:collapse}, almost every outcome $\bx$ of the random zoom causes $L$ to collapse to a function with very \emph{low} variance, and hence the convex body $\zoom{L}{\lambda}{\bx}$ has Gaussian volume very close to either 0 or 1.

\end{itemize}

This means that ``zoom outcome by zoom outcome'', $\zoom{L}{\lambda}{\bx}$ is typically a  very poor approximator for $\zoom{K}{\lambda}{\bx}$; it follows (formally, by \Cref{obs:completion-to-Gaussian}) that $L$ must overall be a very poor approximator for $K$.

We now proceed with the formal proof. 

\medskip

\noindent \emph{Proof of \Cref{thm:high-GNS-hard}.} 
Let $K \subset \R^n$ be a convex set with $\GNS_{n^{-c_1}} \geq {\frac 1 2} - n^{-c_2}.$
By \Cref{lem:expected-variance}, we have
\[
\Ex_{\bx}\sbra{
\Var_{\by}\sbra{
\zoom{K}{2n^{-c_1}}{\bx}(\by)
}
}
\geq 1 - 2n^{-c_2}.
\]
Since $\Var_{\by}\sbra{\zoom{K}{2n^{-c_1}}{\bx}(\by)} \in [0,1]$ for all outcomes of $\bx$, a standard reverse Markov argument gives that
\[
\Prx_{\bx}\sbra{
\Var_{\by}\sbra{
\zoom{K}{2n^{-c_1}}{\bx}(\by)
}
\geq 1 - \sqrt{2}n^{-c_2/2}}
\geq 1 - \sqrt{2}n^{-c_2/2}.
\]
Consequently, for at least a $1 - \sqrt{2}n^{-c_2/2}$ fraction of outcomes of $\bx$, we have that
\begin{equation} \label{eq:firstie}
\Prx_{\by}\sbra{
\zoom{K}{2n^{-c_1}}{\bx}(\by) = 1
} \in \sbra{{\frac 1 2} - 2^{1/4}n^{-c_2/4},{\frac 1 2} + 2^{1/4}n^{-c_2/4}}.
\end{equation}

On the other hand let $L$ be any intersection of at most $2^{\Theta(n^{2c_1/49})}$ many halfspaces over $\R^n$.  
By \Cref{cor:polytope-collapse} (with its $\delta = 1/\log k = n^{-2c_1/49}$), we get that 
\[
\Prx_{\bx \sim N(0,I_n)} \sbra{\Var\pbra{\zoom{L}{\lambda}{\bx}} \geq n^{-2c_1/49}} \leq n^{-2c_1/49}.
\]
So for a least a $1 - n^{-2c_1/49}$ fraction of outcomes of $\bx$, we have that
\begin{equation} \label{eq:secondie}
\min \cbra{\Prx_{\by}\sbra{\zoom{L}{\lambda}{\bx}(\by)=1},\Prx_{\by}\sbra{\zoom{L}{\lambda}{\bx}(\by)=-1}} \leq n^{-2c_1/49}.
\end{equation}
Combining \Cref{eq:firstie} and \Cref{eq:secondie}, for at least a $1 - \max\{\sqrt{2}n^{-c_2/2},n^{-2c_1/49}\}$ fraction of outcomes of $\bx$, we have that
\[
\abs{
\Prx_{\by}\sbra{
\zoom{K}{2n^{-c_1}}{\bx}(\by)=1} 
-
\Prx_{\by}\sbra{\zoom{L}{\lambda}{\bx}(\by)=1
}
} 
\geq
{\frac 1 2} - 2^{1/4}n^{-c_2/4} - n^{-2c_1/49}.
\]
Applying \Cref{obs:completion-to-Gaussian}, we get that
\[
\Vol(K \ \triangle L) \geq 
\pbra{{\frac 1 2} - 2^{1/4}n^{-c_2/4} - n^{-2c_1/49}} \cdot
\pbra{1 - \max\{\sqrt{2}n^{-c_2/2},n^{-2c_1/49}\}},
\]
and the theorem is proved.
\qed



\subsection{Existence of convex sets with high Gaussian noise sensitivity at low noise rates}
\label{sec:existence} 

In this subsection we argue that there exist convex sets with the desired high Gaussian noise sensitivity at low noise rates.  

\red{(I think the following ``theorem'' is the statement that would give us convex sets with the desired high Gaussian noise sensitivity at very low noise rates -- is the ``theorem'' statement true?  Will the convex-Nazarov project prove this? 
In the rest of this subsection after the ``theorem'' statement I'll justify why it would give us what we want.)}
\begin{theorem} \label{thm:highGNS}
There is a convex set $K \subset \R^n$ with the following properties:

\begin{enumerate}

\item $K$ is an intersection of finitely many halfspaces, i.e.~$K=H_1 \wedge \cdots \wedge H_N$, the $i$-th of which is at some Euclidean distance $r_i \leq 2n^{1/4}$ from the origin and includes the origin;

\item We have
\[
\Prx_{\bz \sim N(0,I_n)}[\text{(i) and (ii)}] \geq 1/2 - n^{-a},
\]
where (i) is the event that $\bz \in K$ and $\|\bz\|_2 \leq 2\sqrt{n}$, and (ii) is the event that there exists a $j \in [N]$ such that $\bz$ is at Euclidean distance at most $n^{-b}$ from the hyperplane defining $H_j$. (Here $a>0,b>1/4$ are absolute constants.)\rnote{Can we get this with $b>1/4$? I'm worried that this may be too much to hope for because of $n^{1/4}$ upper bound on noise sensitivity...}

\end{enumerate}
\end{theorem}

Let us explain why a convex set $K$ with the properties of \Cref{thm:highGNS} will have $\GNS_{n^{-c_1}}(K) \geq {\frac 1 2} - n^{-c_2}$ for some constants $c_1,c_2.$
So, let $K$ be as in \Cref{thm:highGNS}.
Let $(\bz,\bz')$ be a pair of $(1-2n^{-c_1})$-correlated $N(0,I_n)$ Gaussians.
Fix $z$ to be any outcome of $\bz$ satisfing conditions (i) and (ii) of Item~(2) of \Cref{thm:highGNS}.
For simplicity, let $e_1$ denote the direction of the orthogonal vector for the hyperplane $H_j$ from condition (ii) for $z$ (this is wlog by Gaussian rotational symmetry).
We have that $\bz'$ is distributed as $(1-2n^{-c_1})z_1 + \sqrt{4n^{-c_1} - 4n^{-2c_1}} \bg$, and by (ii) we know that $z_1 \geq r_j - n^{-b}$, where $r_j$ is at most $2n^{1/4}$ .
So $\bz'_1 \geq r_j$ (and hence $f(\bz') = -1$) if
\[
\pbra{1-2n^{-c_1}}\pbra{r_j - n^{-b}} + \sqrt{4n^{-c_1} - 4n^{-2c_1}} \bg \geq r_j,
\]
Using $r_j \leq 2n^{1/4}$, we get that
\begin{align*}
\Prx[f(\bz') = -1]
&\geq
\Prx\sbra{
\sqrt{4n^{-c_1} - 4n^{-2c_1}}\bg \geq 2n^{-c_1} \cdot 2n^{1/4} + n^{-b}
}\\
&= \Prx \sbra{\bg \geq {\frac {4n^{-c_1 + 1/4} + n^{-b}}{\sqrt{4n^{-c_1} - 4n^{-2c_1}}}}}\\
&\red{\approx}
\Pr\sbra{
\bg \geq 2n^{-c_1/2 + 1/4} + n^{-b + c_1/2}}.
\end{align*}
We take $c_1=1/2 + 2a$ and $b=1/4+2a$, and we get
\[
\Prx\sbra{f(\bz') = -1} \geq \Prx\sbra{\bg \geq \Theta(n^{-a})} = 1/2 - \Theta(n^{-a}).
\]
Recalling that a $1/2 - n^{-a}$ fraction of outcomes of $\bz$ satisfy (i) and (ii), we see that
\[
\Prx_{\bz,\bz'}\sbra{
f(\bz) = 1, f(\bz') = -1
}
\geq \pbra{1/2 - n^{-a}}\pbra{1/2 - \Theta(n^{-a})}=1/4 - \Theta(n^{-a}).
\]
Consequently $\GNS_{n^{-c_1}} = 2\Prx_{\bz,\bz'}\sbra{f(\bz) = 1, f(\bz') = -1} \geq 1/2 - \Theta(n^{-a})$
as was to be shown.

\newpage



==> sections/shivam-10-29-intro-conflict.tex <==
%!TEX root = ../polytope-approximation.tex

\section{Introduction} \label{sec:intro}

A long line of mathematical research has investigated \emph{convex polyhedral approximation of convex bodies}, i.e. the broad question of how to best approximate general  convex bodies using intersections of halfspaces (or equivalently, convex hulls of finite point sets).
Research on questions of this sort dates back at least to the first half of the twentieth century, see for example the early works of Sas \cite{Sas39}, Fejes T\'{o}th \cite{FejesToth48} and Macbeath \cite{Macbeath51}, among others.  
Contemporary motivation for the study of polyhedral approximation of convex bodies arises from many areas including discrete and computational geometry, geometric convexity, the study of finite-dimensional normed spaces, and optimization. 
Given this breadth of connections, it is not surprising that the existing body of work on the subject is vast, as witnessed by the hundreds of references that appear in multiple surveys (including the 1983 \cite{Gruber83} and 1993 \cite{Gruber93} surveys of Gruber and the 2008 survey of Bronstein \cite{Bronstein08})
on approximation of convex bodies by polyhedra.

In the polyhedral approximation literature to date, a number of different distance notions have been used to measure the accuracy of convex polyhedral approximations of convex sets. 
These include the Hausdorff distance, the Nikodym metric (volume of the symmetric difference), the Banach-Mazur distance, distances generated by various $L_p$ metrics, and more.  
(See \cite{Bronstein08} for descriptions of each of these metrics and for an extensive overview of approximability results under each of those distance measures.)

This paper adopts a new perspective, by considering approximation of convex bodies in $\R^n$ using the \emph{(standard) Gaussian volume of the symmetric difference} as the distance measure. 
We refer to this distance measure simply as the \emph{Gaussian distance}. 
This is a natural and well-studied distance measure in theoretical computer science, as witnessed by the many works that have considered learning, testing, derandomization, and other problems using it (see e.g. \cite{KOS:08,Vempalafocs10,MORS:10,Kane:Gotsman11,Kane12,Kane14,KK14,KNOW14,Kane15,CDS19,DMN19,DKPV21,OSTK21,DMN21,HSSV22,DNS23-convex}\rnote{These are learning/testing/derandomization papers; should we add sampling/integration to the list of topics in the sentence, and add references to Santoshy papers on that stuff?  Is it legit to describe it as connected to Gaussian distance?}  and references therein). Given this body of work, it is perhaps surprising that Gaussian distance does not appear to have been previously studied in a systematic way for the convex polyhedral approximation problem.
%\rnote{Are we okay with saying this? I'm sure some works at least mentioned generalizing symmetric difference distance to other measures besides Lebesgue, for instance Boroczky \cite{Boroczky00} mentions that the symmetric difference metric can be generalized by integrating a positive continuous function over the symmetric difference. But he doesn't really do anything with this observation I think, and in particular doesn't do anything Gaussian-specific.  Let's think about how to phrase the claim of novelty...}. 

Let us make our notion of approximation precise:

\begin{definition}  \label{def:Gaussian-volume}
Given (measurable) sets $K,L \subseteq \R^n$, we define the \emph{Gaussian distance} between $K$ and $L$ to be
\[
	\dG(K,L) %= \Vol(K \, \triangle \, L) 
	:= \Prx_{\bx \sim N(0,I_n)}\sbra{\bx \in K \, \triangle \, L}.
\]
\end{definition}

We consider approximators which are intersections of finitely many $n$-dimensional halfspaces, and we measure the complexity of such an approximator by the number of halfspaces (facets) that it contains; we refer to this as its \emph{facet complexity}.
Thus, we are concerned with the following broad question:  

\begin{quote}
Given a convex set $K$ in $\R^n$ and a value $0 < \eps < 1/2$, what is the minimum 
facet complexity of an intersection of halfspaces $L$ 
%number $N$ such that there is some intersection of $N$ halfspaces (which we denote $L$) 
such that $\dG(K, L) \leq \eps$?  
\end{quote}

\subsection{Motivation}

The broad approximation question stated above arises naturally in the context of contemporary theoretical computer science.  As alluded to earlier, an increasing number of results across different areas of TCS involve convex sets and the Gaussian distance;  taking the next step on various natural problems in these areas would seem to require an understanding of how well intersections of halfspaces can approximate convex sets in $\R^n$.  We give two specific examples below:

\begin{itemize}

\item \textbf{Testing Convex Sets:}  A number of researchers have considered the property testing problem of efficiently determining whether an unknown set $K \subseteq \R^n$ is convex versus far from convex \cite{RV04,CFSS17,BBB20,BB20,BBH23}. The Gaussian distance provides a  clean mathematical framework for this problem, and one in which a natural analogy emerges between the well-studied problem of monotonicity testing over the Boolean hypercube and convexity testing \cite{CDNSW23inprep}. Understanding how convex sets can be approximated by ``simpler objects'' under the Gaussian distance seems likely to be helpful in developing algorithms for testing convexity.  (In support of this thesis, we recall that the study of approximating linear threshold functions by ``simpler objects'' \cite{Servedio:07cc} yielded insights and technical ingredients, namely the notion of the ``critical index,'' that played an essential role in the development of efficient algorithms for testing linear threshold functions \cite{MORS:10}.) We also recall that several papers have given testing algorithms for single halfspaces \cite{MORS:10} and intersections of $k$ halfspaces \cite{DNS23-convex} over $\R^n$ under the Gaussian distance; combining these results with results about approximating general convex sets by intersections of halfspaces offers a potential avenue to developing testers for general convex sets.

\item \textbf{Properly Learning Convex Sets:} It has long been known \cite{BshoutyTamon:96} that monotone Boolean functions over $\{-1,1\}^n$ can be learned to any constant accuracy under the uniform distribution in time $2^{\tilde{O}(\sqrt{n})}$, via the ``low-degree'' algorithm based on the Fourier decomposition. Similarly, it has been known for some time \cite{KOS:08} that convex sets can be learned to any constant accuracy under the Gaussian distance, via a ``Hermite polynomial'' variant of the low-degree algorithm.  However, neither the algorithms of \cite{BshoutyTamon:96} nor \cite{KOS:08} are \emph{proper}: in the monotone case the output hypothesis of the learning algorithm is not a monotone function, and in the convex setting the output hypothesis is not a convex set.  Exciting recent work \cite{LRV22} has given a $2^{\tilde{O}(\sqrt{n})}$-time uniform-distribution learning algorithm for monotone Boolean functions over $\{-1,1\}^n$ that \emph{is} proper (even in the demanding \emph{agnostic learning} model, see \cite{LV23}); given this, it is a natural goal to seek a $2^{\tilde{O}(\sqrt{n})}$-time proper learning algorithm for convex sets under the Gaussian distance.  What would the output hypothesis of such a hoped-for proper learning algorithm look like? It seems quite plausible that it would be an intersection of halfspaces; this begs the question of understanding the capabilities and limitations of intersections of halfspaces as approximators for general convex sets in $\R^n$.

\end{itemize}


We further note that intersections of halfspaces have been intensively studied in many branches of ``concrete complexity theory;'' indeed, many of the TCS results alluded to earlier that involve Gaussian distance are more specifically about intersections of halfspaces, e.g. \cite{KOS:08,Vempalafocs10,CDS19,DMN19,DKPV21,DMN21,HSSV22}. 
%So it is natural to study the extent to which intersections of halfspaces can approximate more general convex sets.

Finally, we note that the suite of tools which turn out to be relevant in our study link our investigations closely to theoretical computer science.  Perhaps unexpectedly, we will see that there are close connections between the study of facet complexity of polyhedral convex approximators and a number of fundamental ingredients and results (such as noise sensitivity, random restrictions, influence of variables/directions, various extremal constructions, etc.) in the \emph{analysis of Boolean functions} over the discrete domain $\{-1,1\}^n$.  From this perspective, our study can be seen as a continuation of the broad theme of exploring the emerging analogy between convex sets in $\R^n$ under the Gaussian distribution and monotone Boolean functions over $\{-1,1\}^n$ under the uniform distribution (see e.g.~\cite{DS21colt,DNS21itcs,DNS22,HSSV22}).

%\gray{\emph{This regime is of interest to TCS.  Facet complexity is equivalent to size as an intersection of halfspaces, which is well studied in TCS. Indeed many of our tools come from TCS (noise sensitivity, random restrictions, influences of variables/coordinates), though we also use ideas and results from math results on other notions of approximation (Hausdorff, etc).}
 
%\emph{A number of works in TCS have studied algorithmic problems having to do with convex sets and intersections of halfspaces under the Gaussian distribution (examples: random sampling stuff; convex set learning and testing; etc).  Understanding the approximability of convex sets in this setting can be useful for future work there.  (Maybe talk about a convex sets analogue of Lange/Rubinfeld/Vasiliyan as a goal result, towards which it'd be good to understand the approximation questions we consider.)}

\rnote{I didn't mention \href{http://proceedings.mlr.press/v65/diakonikolas17a/diakonikolas17a.pdf}{http://proceedings.mlr.press/v65/diakonikolas17a/diakonikolas17a.pdf}, which uses polytope approximation (w.r.t. Lebesgue, right?) for some distribution learning thing --- is there a natural way to mention it?
}

\medskip

Before turning to an overview of our results and techniques, let us fix some convenient notation and terminology.  If $L \subseteq \R^n$ is an intersection of $N$ halfspaces, then as stated earlier we say that the \emph{facet complexity} of $L$ is $N$, \red{and we write this as $\FC(L)=N$}\rnote{Will we ever use this? If not let's delete?}. Given a convex set $K \subseteq \R^n$ and a value $0 \leq \eps < 1/2$, we write $\FC(K,\eps)$ to denote the minimum value $N$ such that there is a convex set $L$ with $\FC(L)=N$ (i.e. $L$ is an intersection of $N$ halfspaces) satisfying $\dG(K,L) \leq \eps.$

%\rnote{Let's have a longish section in which we describe all of the results, interspersed with high-level explanations of the techniques. and explain how they relate to each other. Then the later sections can  more or less just give the proofs and intuitions of the proofs.}

\section{Overview of Results and Techniques}


\begin{table}[]
\centering
\renewcommand{\arraystretch}{1.25}
\red{
\begin{tabular}{@{}llll@{}}	
\toprule
Convex $K \sse\R^n$ & $\eps$        & Upper Bound                                                          & Lower Bound                                                                 \\ \midrule\midrule
Arbitrary $K$ with $\Vol(K) = \delta$ & $0.01$                             & \begin{tabular}[t]{@{}l@{}}$\frac{1}{\delta} \cdot \pbra{n\log\pbra{\frac{1}{\delta}}}^{O(n)}$ \\[-0.1em] (\Cref{thm:rel-err-dud})  \end{tabular} & \hfill---~~~~~~~~                                                                                        \\ \midrule
$\ell_2$-ball of Gaussian measure $1/2$          & $0.01$                        & \begin{tabular}[t]{@{}l@{}}$2^{O(\sqrt{n})}$ \\[-0.25em] (\Cref{thm:de-nazarov}) \end{tabular} & \begin{tabular}[t]{@{}l@{}}$2^{\Omega(\sqrt{n})}$ \\[-0.25em] (\Cref{thm:high-influence-lb}) \end{tabular}                                        \\\midrule
$\ell_1$-ball of Gaussian measure $1/2$          & $0.01$                        & \begin{tabular}[t]{@{}l@{}}$2^{O(n^{3/4})}$ halfspaces \\[-0.25em] (\Cref{thm:ell-1-approx}) \end{tabular}  & \begin{tabular}[t]{@{}l@{}}$2^{\Omega(\sqrt{n})}$ \\[-0.25em] (\Cref{thm:high-influence-lb}) \end{tabular}                                       \\ \midrule
$K$ s.t. $\GNS_{\frac{1}{\poly(n)}}(K) \geq \frac{1}{2} - \frac{1}{\poly(n)}$~~ &  ${\frac{1}{2} - \frac{1}{\poly(n)}}$                                                                 & ~~~~~~~~~---~~~      & \begin{tabular}[t]{@{}l@{}}$2^{n^{\Omega(1)}}$ \\[-0.25em] (\Cref{thm:high-GNS-hard}) \end{tabular} \\ \bottomrule
\end{tabular}
}
\caption{A partial summary of our bounds on the facet complexity $\FC(K,\eps)$ for convex sets.}
\label{tab:results}
\end{table}


We now turn to a technical overview of our results. A partial summary of some of our main results is presented above in~\Cref{tab:results}. 

\subsection{Overview of Positive Results}

We start with our positive results on approximability of convex sets under the Gaussian distance by intersections of halfspaces. 

\paragraph{Universal Approximation via Hausdorff Distance Approximation.}  As a warmup, we begin in \Cref{subsec:dudley} by giving a fairly simple ``universal approximation'' result that upper bounds $\FC(K,\eps)$ for any convex set $K \subseteq \R^n$.  The key observation (implicit in the proof of \Cref{thm:gaussian-dudley}) is that for any convex set $K$, if $L$ is an intersection of halfspaces which is a high-accuracy \emph{outer}\footnote{Recall that $L$ is an \emph{outer} (respectively \emph{inner}) approximator to $K$ if $K\sse L$ (respectively $L\sse K$).} approximator of $K$ under the Hausdorff distance measure, then $L$ is also a (slightly lower accuracy) $\dG$-approximator for $K$.  (Recall that the Hausdorff distance between two sets $S,T \subseteq \R^n$ is $\max\cbra{\sup_{s \in S}\|s-T\|, \sup_{t \in S}\|t - S\|}$, where $\|x-Y\| = \inf_{y \in Y}\|x-y\|$ and $\|x-y\|$ is the Euclidean distance between $x$ and $y$.)  This is easy to establish by simply integrating Keith Ball's universal $O(n^{1/4})$ upper bound \cite{Ball:93} on the \emph{Gaussian surface area} of any convex set (see \Cref{thm:ball}), using the fact that for any $t > 0$ and any convex set $K$, the ``$t$-enlargement'' $K_t$ of $K$ is also a convex set (see the proof of \Cref{thm:gaussian-dudley}).

Combining the above observation with standard Gaussian tail bounds and classical upper bounds on the facet complexity of an outer Hausdorff approximator for any convex body with bounded radius, we obtain the following:

\begin{theorem} [Informal version of \Cref{thm:gaussian-dudley}.] \label{thm:gaussian-dudley-informal}
For any convex set $K$ and any $\eps > 0$, we have $\FC(K,\eps) \leq (n/\eps)^{O(n)}.$
\end{theorem}

\paragraph{A ``Relative-Error'' Universal Approximation Sharpening of \Cref{thm:gaussian-dudley-informal}.}  Suppose that $K \subseteq \R^n$ is a convex set whose Gaussian volume is very large, i.e.~$1-\delta$ where $\delta$ is very small.  In this situation the trivial approximator which is all of $\R^n$ already has $\dG(K,\R^n)=\delta$, so a natural goal for approximation is to achieve small error \emph{relative to} the $\delta$ amount of mass which lies outside of $K$, i.e. to construct an intersection of halfspaces $L$ for which 
\[\dG(K,L) \leq \eps \delta.\]  
While \Cref{thm:gaussian-dudley-informal} shows that $(n/(\eps \delta))^{O(n)}$ halfspaces suffice for this, in \Cref{subsec:good-dudley} we give a stronger result which has a significantly improved dependence on $\delta$:

\begin{theorem} [Informal version of \Cref{thm:rel-err-dud}.]
\label{thm:rel-err-dud-informal}
Let $0<\eps,\delta<1$ and let $K \subsetneq \R^n$ be a  convex set with 
$\Vol(K) = 1-\delta.$  Then 
\[\FC(K,\eps \delta) \leq 
%	\[ \frac{8}{\eps\delta}\log\pbra{\frac{4}{\eps\delta}}\pbra{\frac{2000}{\eps}\pbra{\sqrt{n} + 2\sqrt{\ln\pbra{\frac{2}{\eps\delta}}}}}^{3n}= \frac{8}{\eps\delta}\log\pbra{\frac{4}{\eps\delta}}O\pbra{\frac{n}{\eps}\log\pbra{\frac{1}{\delta}}}^{O(n)}~\text{halfspaces}\]
\frac{1}{\delta} \cdot \pbra{\frac{n}{\eps}\log\pbra{\frac{1}{\delta}}}^{O(n)}.
\]
\end{theorem}

\noindent 
(We remark that the strengthening which \Cref{thm:rel-err-dud} achieves over \Cref{thm:gaussian-dudley} will be crucial for the construction of our $\ell_p$-ball approximators, discussed below.)

We briefly explain the main idea underlying the construction of the approximator  of \Cref{thm:rel-err-dud}.  First, we recall a basic property of the $N(0,I_n)$ distribution, which is that along any ray $\{tv: t \geq 0\}$ from the origin in $\R^n$, the distribution of Gaussian mass along that ray follows the chi-distribution (see \Cref{subsec:prelims-gaussian}).  Since $\Vol(K)=1-\delta$, this means that the ``amount of chi-distribution mass'' which is ``lopped off'' by $K$ along direction $v$, averaged over all directions $v$, is $\delta$.  The high-level idea of our construction of the approximator $L$ is to place tangent hyperplanes on the boundary of $K$ in such a way as to ``lop off'' {at least a} $(1-\eps)$-fraction of the total $\delta$ amount of Gaussian mass that lies outside the set $K$. We do this via an analysis that proceeds direction by direction: We can ignore directions in which $K$ ``lops off'' only a very small amount (less than $\eps \delta/4$, say) of the chi-distribution's mass. For the other directions, we use a bucketing scheme, a suitable net construction for the points in each bucket, and a mixture of careful geometric arguments and tail bounds to argue that not too many halfspaces are required to adequately handle all of the other directions.

\paragraph{\bf Sub-Exponential Approximation for Specific Convex Sets.}
Going beyond the universal approximation results mentioned above, it is natural to wonder whether improved approximation bounds can be obtained for specific interesting convex sets.
Perhaps the two most natural convex sets to consider in this context are the $\ell_1$ and $\ell_2$ balls\footnote{Observe that the $\ell_\infty$ ball $\cbra{x \in \R^n \ : \ \|x\|_\infty \leq r}$ is an intersection of $2n$ halfspaces $-r \leq x_i \leq r, i \in [n]$. \shivam{Should this be a footnote about the $\ell_1$ ball? It seemed a little out of place to me otherwise.}} of Gaussian volume $1/2$, which we briefly discuss below.
  
The $\ell_1$ ball of Gaussian volume $1/2$, also known as the ``spectrahedron'' or ``cross-polytope,'' is the convex set 
%\rnote{I don't love this $B_1(1/2)$ notation for the $\ell_1$ ball of volume $1/2$, since we're writing $B(\sqrt{n})$ to denote the $\ell_2$ ball of radius $\sqrt{n}$; any suggestions?}
\[
 \cbra{x \in \R^n \ : \|x\|_1 \leq c n},
\]
where $c = \sqrt{2/\pi} \pm o_n(1)$ (this is an easy consequence of the Berry-Esseen theorem).  This set is an intersection of exactly $2^n$ halfspaces, namely
\[
 b_1 x_1 + \cdots + b_n x_n \leq c n
\text{~for all~}(b_1,\dots,b_n) \in \{-1,1\}^n,
\]
and it is natural to wonder whether this set can be approximated as an intersection of significantly fewer than $2^n$ halfspaces.  

The $\ell_2$ ball of Gaussian volume $1/2$ is simply the Euclidean ball
\[
\cbra{ x \in \R^n \ : \|x\|^2 \leq \text{median}(\chi^2(n))}.
\]
(Of course, writing this set \emph{exactly} as an intersection of halfspaces requires infinitely many halfspaces.)
Using well-known bounds on the chi-squared distribution we have that the Euclidean ball of radius $1/2$, which we denote $B(\sqrt{n})$, has Gaussian volume $1/2 + o_n(1)$; it will be slightly more convenient for us to use this as the $\ell_2$ ball that we seek to approximate. 

\medskip

\noindent {\bf A 
%$2^{\tilde{O}(1/\eps) \cdot \sqrt{n}}$-facet 
$2^{O(\sqrt{n})}$-facet 
approximator for the $\ell_2$-ball.}
For several standard distance measures, including the Hausdorff distance and the symmetric-difference measure, the $\ell_2$-ball is the ``hardest case'' for approximation by  intersections of halfspaces, matching or essentially matching known upper bounds for universal approximation.  For example, it is known \cite{Bronstein08} that any intersection of halfspaces which is an $\eps$-approximator to $B(\sqrt{n})$ in Hausdorff distance must have facet complexity $\Omega((\sqrt{n}/\eps)^{(n-1)/2})$, matching the universal approximation upper bound for Hausdorff distance to within a constant factor \cite{AFM12}.
For the symmetric-difference measure, Ludwig, Sch\"{u}tt and Werner \cite{LSW06} showed that if $L$ is an intersection of $M$ halfspaces for which \red{${\frac {\mathrm{Leb}(L \ \triangle \ B(\sqrt{n}))}{\mathrm{Leb}(B(\sqrt{n}))}} \leq c$ (here $\mathrm{Leb}$ denotes volume under the standard Lebesgue measure)}\rnote{Is this notation what we want to use for Lebesgue?}, where $c>0$ is some absolute constant, then $M$ must be at least $2^{\Omega(n)}$.

In contrast, for the Gaussian distance we are able to exploit the rotational symmetry of the standard Gaussian distribution and tail bounds on the chi-distribution to get an approximation of the $\ell_2$ ball which uses much fewer than $2^n$ facets, and hence is much better than the universal approximation upper bounds given by \Cref{thm:gaussian-dudley-informal} or \Cref{thm:rel-err-dud-informal}.  For any constant $\eps$, we give a probabilistic construction of a $2^{O(\sqrt{n})}$-facet polytope which is an $\eps$-approximator of the $\ell_2$ ball.  This construction is analogous to a probabilistic construction of O'Donnell and Wimmer \cite{o2007approximation}, which shows that a variant of a random monotone CNF construction due to Talagrand \cite{Talagrand:96} gives an $\eps$-accurate approximator for the Boolean Majority function.  We similarly modify  a probabilistic construction of a convex body due to Nazarov~\cite{Nazarov:03}, and use it to prove the following in \Cref{sec:nazarov-ub}:

\begin{theorem} [Informal version of \Cref{thm:de-nazarov}.]
\label{thm:de-nazarov-informal}
Let $B$ denote the $\ell_2$-ball of radius $\sqrt{n}$ in $\R^n$ (so $\Vol(B) = 1/2 + o_n(1)$). Then 
$\FC(B,\eps) \leq 2^{\tilde{O}(1/\eps) \cdot \sqrt{n}}.$
\end{theorem}


\noindent {\bf A $2^{O(n^{3/4})}$-facet approximator for the $\ell_1$-ball.} 
Since the $\ell_1$ ball does not enjoy the same level of rotational symmetry as the $\ell_2$ ball, it is natural to wonder whether it can be similarly approximated with a sub-exponential number of facets. \rnote{Do we want to go into this whole story? I think otherwise it might seem a little unmotivated for us to be studying the $\ell_1$ ball...}As we now explain, another motivation for this question comes from considering a result of O'Donnell and Wimmer on the inability of small CNF formulas to approximate the ``tribes'' Boolean DNF formula over $\zo^n$, in the context of a  recently-explored analogy between monotone Boolean functions and symmetric convex sets~\cite{DS21colt,DNS21itcs,DNS22,HSSV22}. 

In \cite{o2007approximation} O'Donnell and Wimmer showed that any CNF formula that computes the $n$-variable DNF tribes function correctly on $(1-\eps) \cdot 2^n$ inputs, for $\eps = 0.1$, must have $2^{\Omega(n/\log n)}$ clauses.  As detailed in \cite{DS21colt,DNS22}, there is a natural correspondence between $s$-clause CNF formulas over $\{0,1\}^n$ and symmetric intersections of $2s$ halfspaces over $N(0,I_n)$ (this correspondence is at the heart of the main lower bound of \cite{DS21colt} and several of the results of \cite{HSSV22,DNS22}).  Thus, in seeking convex sets that may require $2^{\tilde{\Omega}(n)}$ halfspaces to approximate under $N(0,1)^n$, it is natural to look for a Gaussian space convex analogue of of the DNF tribes function over $\{0,1\}^n$.  Now, 
\begin{itemize}

\item the DNF tribes function is the Boolean dual of the CNF Tribes function; 
\item the Gaussian-space polytope corresponding to the CNF Tribes function is the $\ell_\infty$ ball \cite{DNS22,HSSV22}; and 
\item the polytope which is dual to the $\ell_\infty$ ball is the $\ell_1$ ball.  

\end{itemize}
Thus the  following question naturally suggests itself:  does the $\ell_1$ ball in $\R^n$ of volume $1/2$ under $N(0,I_n)$ require $2^{\tilde{\Omega}(n)}$ halfspaces for constant-accuracy approximation, analogous to how the DNF Tribes function requires $2^{\tilde{\Omega}(n)}$-clause CNFs for constant-accuracy approximation?

%The rotational symmetry of the standard Gaussian distribution aligns perfectly with the rotational symmetry of the $\ell_2$ ball.  While the $\ell_1$ ball is not as rotationally symmetric as the $\ell_2$ ball, we  

While the above conjecture may seem intuitively plausible (and indeed, the authors initially tried to prove it), it turns out to be false. In \Cref{subsec:ell-1-warmup} we show that the $\ell_1$ ball can be approximated to any constant accuracy as an intersection of sub-exponentially many halfspaces:

\begin{theorem} [Informal version of \Cref{thm:ell-1-approx}.]
\label{thm:ell-1-approx-informal}
Let $\CP$ denote the origin-centered $\ell_1$-ball in $\R^n$ with $\Vol(\CP)=1/2.$  Then $\FC(\CP,\eps) \leq
2^{\tilde{O}(1/\eps^{3/2}) \cdot n^{3/4}}.$
\end{theorem}

We prove \Cref{thm:ell-1-approx-informal} using a probabilistic construction, but one which is very different from the probabilistic construction described above in the sketch of \Cref{thm:de-nazarov-informal} for the $\ell_2$ ball.  The high-level intuition is as follows:  Determining whether or not a point $x \in \R^n$ lies within $\CP$ is the same as determining whether or not the sum $|x_1| + |x_2| + \dots + |x_n|$ exceeds the correct threshold (which is roughly $\sqrt{2/\pi}n$).  Given this, the main idea is to take a probabilistic approach which exploits both \emph{anti-concentration} and \emph{sampling}: 

\begin{itemize}

\item  Anti-concentration tells us that for $\bx \sim N(0,I_n)$, only a small fraction of outcomes of $|\bx_1|+\cdots + |\bx_n|$ will lie very close to the boundary value of $\sqrt{2/\pi}n$.  Thus, at the cost of a small error, we can assume that a typical outcome $x$ of $\bx$ either has $|x_1| + \cdots + |x_n| \geq \sqrt{2/\pi}n + \tau$ (call this a ``heavy'' $x$), or has $|x_1| + \cdots + |x_n| \leq \sqrt{2/\pi}n - \tau$ (call this a ``light'' $x$) for a suitable margin parameter $\tau$. 

\item Given this, we can use a sampling-based approach:   if we uniformly sample $r$ coordinates $\bi_1,\dots,\bi_r$ from $[n]$ and evaluate $|x_{\bi_1}| + \cdots + |x_{\bi_r}|$, then for a suitable threshold $\theta_1$ there will be a noticeable gap between (i) the (extremely large) probability that $|x_{\bi_1}| + \cdots + |x_{\bi_r}| \geq \theta_1$ when $x$ is a typical heavy point, and  (ii) the (still very large, but slightly smaller) probability that $|x_{\bi_1}| + \cdots + |x_{\bi_r}| \geq \theta_1$ when $x$ is a typical light point.

\end{itemize} 

The above gap means that by ANDing together a carefully chosen number $M$ of random sets of the form
\begin{equation}
\cbra{x \in \R^n \ : \ |x_{\bi_1}| + \cdots + |x_{\bi_r}| \geq \theta_1},\label{eq:juntaell1}
\end{equation}
we get an approximator for $\CP$ which is accurate on almost all of the points $x \in \R^n$ which are either light or heavy (and, as sketched above, almost all points drawn from $N(0,I_n)$ are either light or heavy, by anti-concentration). The detailed analysis requires sophisticated Cram\'{e}r-type bounds which give very tight \emph{multiplicative} control on tails of sums of random variables drawn \emph{without} replacement from a finite population of values.



 Note that each set of the form (\ref{eq:juntaell1}) is an $r$-variable ``junta'' $\ell_1$ ball over its $r$ relevant coordinates (and is also an intersection of $2^r$ halfspaces), so the AND of $M$ such sets is an intersection of $M2^r$ many halfspaces.  With careful balancing of parameters we get that this is at most $2^{O(n^{3/4})}$ halfspaces, for any constant-factor approximation.

\medskip

\noindent {\bf A $\red{2^{n^{3/4} \text{~or something}}}$-facet approximator for the $\ell_p$-ball, $1 \leq p < 2.$} \Cref{thm:de-nazarov-informal} and \Cref{thm:ell-1-approx-informal} give sub-exponential approximators for the $\ell_1$ and $\ell_2$ balls using two different sets of techniques.  We generalize the approach of \Cref{thm:ell-1-approx-informal} to give approximators of similar facet complexity for the $\ell_p$ balls of volume $1/2$, for all $1 \leq p < 2$:

\begin{theorem} [Informal version of \Cref{thm:ell-p-approx}.]
\label{thm:ell-p-approx-informal}
For $1 < p < 2$ let $B_p$ denote the origin-centered $\ell_p$-ball in $\R^n$ with $\Vol(B_p)=1/2.$  Then $\FC(B_p,\eps) \leq \red{2^{n^{3/4}/\eps \text{~or something}}}$.
\end{theorem}

The high-level approach, in its first stage, is similar to the $\ell_1$-ball approximation sketched above.   We now employ anticoncentration of the sum $|\bx_1|^p + \cdots + |\bx_n|^p$, and now in place of random sets of the form (\ref{eq:juntaell1}) we use random sets of the form
\begin{equation} \label{eq:juntaellp}
\cbra{x \in \R^n \ : \ |x_{\bi_1}|^p + \cdots + |x_{\bi_r}|^p \geq \theta_p}
\end{equation}
for a suitable threshold value $\theta_p$.  As before, ANDing together a carefully chosen number $M$ of sets of this form will be a high-accuracy approximator to the volume-$1/2$ $\ell_p$ ball.  But while in the $p=1$ case each set of the form (\ref{eq:juntaell1}) was already an intersection of only $2^r$ halfspaces, for $1<p<2$ a set of the form (\ref{eq:juntaellp}) is not an intersection of any finite number of halfspaces.  Instead, we must replace each set of the form (\ref{eq:juntaellp}) with an intersection of (not too many) halfspaces which is a very high accuracy approximator for it.  Crucially, each set of the form (\ref{eq:juntaellp}) has extremely high volume; this is exactly the setting in which our efficient relative-error approximator, \Cref{thm:rel-err-dud-informal}, is useful.  We apply \Cref{thm:rel-err-dud-informal} to approximate each of the $M$ sets of the form (\ref{eq:juntaellp}) as an intersection of $N$ halfspaces, and then ANDing together all of those approximators we achieve an $MN$-halfspace approximator to the original volume-1/2 $\ell_p$ ball in $\R^n$.

\subsection{Overview of lower bounds}

\noindent {\bf Non-explicit average-case lower bounds.}  It is well known that standard counting arguments easily yield strong (average-case) lower bounds on the complexity of approximating (non-explicit) \emph{Boolean functions} that map $\bn$ to $\bits$. 
For a range of different computational models, these lower bounds show that even achieving approximation error $1/2 - o_n(1)$ requires any approximator to be exponentially large.

In our context of approximating convex sets in $\R^n$ by intersections of halfspaces, counting arguments are not quite as straightforward because there are infinitely many distinct halfspaces over $\R^n$.  Nevertheless, counting arguments can be brought to bear to prove lower bounds. In more detail, \cite{KOS:08} used a counting argument to establish the existence of $N=2^{2^{\Omega(\sqrt{n})}}$ distinct convex sets $K_1,\dots,K_N$ in $\R^n$, each of which is an intersection of $2^{\Omega(\sqrt{n})}$ many halfspaces, such that $\dG(K_i,K_j) \geq 1/44000$ for each $1 \leq i \neq j \leq N.$  Using this result, it is possible to establish the existence of a convex set $K$ (one of the sets $K_1,\dots,K_N$ sets) such that $\FC(K,c) \geq 2^{c \sqrt{n}}$, where $c>0$ is a small absolute constant.

In \Cref{sec:nonexplicit} we give a stronger (but still non-explicit) lower bound, which shows that many halfspaces are required even to achieve error $1/2 - o_n(1)$; in other words, we give an \emph{average-case} lower bound (also known as a \emph{correlation bound}). Our lower bound trades off the accuracy of the approximator against the number of halfspaces:

\begin{theorem} [Informal version of \Cref{lb:non-explicit-convex}.] \label{thm:lb-non-explicit-convex-informal}
For any $\tau = \omega (n^{-1/2} \cdot \log n)$, there exists some convex set $K \subset \mathbb{R}^n$ that has $\FC(K,\frac12 - \tau) = 2^{\Omega(\tau\cdot \sqrt{n})}$.
\end{theorem}

\noindent For example, taking $\tau = n^{-1/4}$, \Cref{thm:lb-non-explicit-convex-informal} implies the existence of an $n$-dimensional convex set $K$ such that no intersection of $2^{cn^{1/4}}$ many halfspaces can approximate $K$ to accuracy even as large as $1/2 + n^{-1/4}$; taking $\tau$ to be a constant, we recover the non-explicit $2^{\Omega(\sqrt{n})}$ lower bound mentioned in the previous paragraph.

The proof of \Cref{thm:lb-non-explicit-convex-informal}  combines classical results from statistical learning theory with an information theoretic lower bound on \emph{weak} learning convex sets under $N(0,I_n)$ that was established in recent work \cite{DS21colt}. The argument proceeds by contradiction:  Suppose that every convex set can be approximated to accuracy $1/2 - \eps$ by an intersection of $M$ halfspaces.  Since there is always an intersection of $M$ halfspaces which is $(1/2-\eps)$-close to any convex set, classical results in statistical learning theory imply that it is information-theoretically possible to \emph{agnostically learn} any unknown convex set $K$ to error $1/2 - \eps/2$, where the learning algorithm uses a number of samples which is essentially) the VC dimension of the class of all intersections of $M$ halfspaces over $\R^n$, i.e.~essentially $O(nM \log M)$.  But a recent result of De and Servedio \cite{DS21colt} implies that any algorithm which ``weak learns'' the entire class of all convex sets over $\R^n$ using at most $S$ samples (or queries) must have error at least essentially $1/2 - \log(S)/\sqrt{n}$. Combining these bounds, it can be shown that $M$ must be at least $2^{\Omega(\eps \cdot \sqrt{n})}$; see \Cref{sec:nonexplicit} for the detailed argument.

The attentive reader may at this point be reminded of an argument from \cite{KKMS:08}, which combined the fact that halfspaces can weakly approximate parity functions with the presumed \emph{computational} hardness of learning noisy parities to obtain evidence that no computationally efficient algorithm exists for agnostically learning halfspaces.  A more recent argument, of perhaps a more similar flavor to the proof of \Cref{thm:lb-non-explicit-convex-informal}, is given in \cite{HSSV22}, where the \cite{DS21colt} result (establishing the non-existence of weak learning algorithms for convex sets with small sample complexity) is used to establish a lower bound on the statistical query complexity of agnostic learning algorithms for intersections of halfspaces. The proof of \Cref{thm:lb-non-explicit-convex-informal} is the first result we know of, though, in which an information-theoretic sample complexity lower bound for weak learning is used to establish an \emph{inapproximability} result.

\medskip

\noindent {\bf Average-case lower bounds via Gaussian noise sensitivity.} 
One drawback of \Cref{thm:lb-non-explicit-convex-informal} is that it is non-constructive: not only does it not exhibit any particular convex set which is hard to approximate, it does not establish any particular criterion that implies that a convex set is hard to approximate.
\Cref{sec:noise-sensitivity} gives such a criterion: we show that any set with very high \emph{Gaussian noise sensitivity} (at least $1/2 - 1/\poly(n)$) at very low noise rates (at most $1/\poly(n)$) requires many halfspaces to approximate to accuracy even $1/2 + 1/\poly(n)$:

\begin{theorem} [Informal version of \Cref{thm:high-GNS-hard}.]
\label{thm:high-GNS-hard-informal}
If $K \subset \R^n$ is any convex set which satisfies $\GNS_{1/\poly(n)}(K) \geq {\frac 1 2} - {\frac 1 {\poly(n)}}$, then $\FC(K,{\frac 1 2} - {\frac 1 {\poly(n)}}) \geq 2^{n^{\Omega(1)}}.$
\end{theorem}

\Cref{thm:high-GNS-hard-informal} naturally raises the question of whether there in fact exist $n$-dimensional convex sets that have Gaussian noise sensitivity as high as $1/2 - 1/\poly(n)$ at noise rates that are as low as $1/\poly(n)$.  While natural, this question does not appear \cite{OD23pc} to have been asked or answered prior to the current work.  In \Cref{sec:existence} we combine the information-theoretic lower bounds of  \cite{DS21colt} on weak learning convex sets with the ``low-degree algorithm'' for learning bounded functions to show that there do exist $n$-dimensional convex sets $K$ with $\GNS_{1/\poly(n)}(K) \geq 1/2 - 1/\poly(n)$ (see \Cref{thm:highGNSlownoise}). We believe that this result may be of independent interest.

The proof of \Cref{thm:high-GNS-hard-informal} combines results from learning theory \cite{KOS:08} and the study of unconditional pseudorandomness \cite{OSTK21} with classical ideas from the study of correlation bounds for Boolean functions \cite{Hastad86,Cai86}.  
It employs a notion of a ``random zoom'' for a function $f: \R^n  \to \R$ which is closely analogous to the well-studied notion of a ``random restriction'' of a function from $\bn$ to $\bn$.

Analogous to the well-known phenomenon that low-depth Boolean circuits over $\bn$ simplify under random restrictions \cite{Hastad86,Cai86}, in the context of developing efficient pseudorandom generators for intersections of halfspaces it was shown in \cite{OSTK21} that low-degree polynomials over $N(0,I_n)$ simplify under random zooms; more precisely, they are very likely to have very low ``hypervariance'' after a random zoom (see \Cref{subsec:zoom-prelims} for detailed definitions).  Moreover, it was shown in \cite{KOS:08} (in the context of developing efficient agnostic learning algorithms for intersections of halfspaces) that any intersection of ``not too many'' halfspaces is close (in a suitable sense) to a low-degree polynomial.  Combining these results, we get that (1) applying a random zoom to any intersection of few halfspaces, we get a function that must have very low hypervariance, and hence must be very close to a constant.  But on the other hand, it can be shown that (2) if a set $K$ has very high Gaussian noise stability at very low noise rates, then after a random zoom it must be very \emph{far} from a constant function.  Similar to classical correlation bounds for shallow Boolean circuits (which use the fact that that the parity function is far from a constant function after random restriction, while shallow Boolean circuits become close-to-constant after random restrictions), the tension between (1) and (2) can be used to deduce that any intersection of ``not too many'' halfspaces must be very far from any set $K$ that has high Gaussian noise stability at low noise rates.

%\red{Say stuff about the proof of \Cref{thm:high-GNS-hard-informal}: uses analogue of random restrictions for Gaussians called random zooms. Crux of the argument is to show that a random zoom of an intersection of ``few'' halfspaces simplifies it very dramatically --- the expected variance after the random zoom is very close to 0, so the set whp becomes close-to-constant.  But if $K$ has very high Gaussian noise sensitivity, then the expected variance of $K$ after the random zoom is $2\GNS_\lambda[K]$, which is very close to 1.  This contradiction shows that no intersection of a small number of halfspaces can be a good approximator, giving \Cref{thm:high-GNS-hard-informal}.}

\medskip

\noindent {\bf Lower bounds via convex influences.}
In \Cref{subsec:convex-influence-lower-bound} we give a different general criterion on a conve set $K \subset \R^n$ which suffices to ensure that $FC(K,\eps) = 2^{\Omega(\sqrt{n})}$, where $\eps$ is a suitable constant.  This criterion is that $K$ has maximal \emph{convex influence}, up to a multiplicative constant factor.  \red{Talk about convex influence: introduced recently, every set has at most thus-and-such, etc}.


\begin{theorem} [Informal version of \Cref{thm:high-influence-lb}.] \label{thm:high-influence-lb-informal}
If $\TInf[K] = \Omega(\sqrt{n})$, then for a suitable constant $\eps>0$ we have that $\FC(K,\eps) = 2^{\Omega(\sqrt{n})}.$
\end{theorem}

\red{Talk about how it's done:  structural result showing that if $L$ is an intersection of $N$ halfspaces then $\TInf[L] = O(\log N).$  (Mention analogue with CNF.)  Parseval.}
 

\medskip

\noindent {\bf Exponential lower bounds for high-accuracy approximators.} Thus far, all of our lower bounds have been at best $2^{\Omega(\sqrt{n})}$ many halfspaces, and have been for achieving either accuracy $1/2 - o_n(1)$ or accuracy $c$ for some constant $0<c<1/2$.  Our last lower bound shows that if we strengthen the accuracy requirement to require error at most $O(1/n)$, then we can achieve a truly exponential lower bound for approximating the $\ell_2$ ball $B(\sqrt{n})$:

\begin{theorem} [Informal version of \Cref{thm:strong-lower-bound}.]
\label{thm:strong-lower-bound-informal}
Let $B$ denote the $\ell_2$-ball of radius $\sqrt{n}$ in $\R^n$ (so $\Vol(B) = 1/2 + o_n(1)$). Then 
\red{$\FC(B,1/n) \leq 2^{\Omega(n)}.$ (fix/check)}
\end{theorem}

\red{Talk about how it's done:  Ludwig-Schutte-Werner etc.}



\gray{* we can translate symmetric-difference-approximation negative results for the ball ("any symmetric-difference- approximator for the ball requires thus-and-such many vertices or facets") to Gaussian-approximation negative results for the ball, for an approximation factor that's a factor of $\sqrt{n}$ worse. (I think the argument only works for the ball, right?)}


\subsection{Discussion}

\blue{Let's have a brief discussion section at the end of the intro. We should raise the $2^{n}$ versus $2^{\sqrt{n}}$ question; other things?}









%\begin{itemize}

%\item \emph{Background: Paragraph or two on how there is a rich line of work in mathematics / high dimensional convex geometry on approximating convex sets in various ways.  (Quick overview of some possibilities for how complexity is measured in prior work:  number of vertices; number of facets; others?  Quick overview of how accuracy is measured in prior work:  Hausdorff distance, Lebesgue distance, Banach-Mazur distance; others?)}

%\item \emph{This work:  We consider a new framework for studying the approximability of convex sets by simpler sets.  Specifically, we study approximating convex sets where (i) we measure complexity of the approximator by the number of facets, and (ii) we measure accuracy w.r.t. the standard $N(0,I_n)$ distribution over $\R^n$.}

%\item \emph{Motivation:  This regime is of interest to TCS.  Facet complexity is equivalent to size as an intersection of halfspaces, which is well studied in TCS. Indeed many of our tools come from TCS (noise sensitivity, random restrictions, influences of variables/coordinates), though we also use ideas and results from math results on other notions of approximation (Hausdorff, etc).}
 
%\emph{A number of works in TCS have studied algorithmic problems having to do with convex sets and intersections of halfspaces under the Gaussian distribution (examples: random sampling stuff; convex set learning and testing; etc).  Understanding the approximability of convex sets in this setting can be useful for future work there.  (Maybe talk about a convex sets analogue of Lange/Rubinfeld/Vasiliyan as a goal result, towards which it'd be good to understand the approximation questions we consider.)}

%\end{itemize}


